Kelly Cache Networks

We study networks of M/M/1 queues in which nodes act as caches that store objects. Exogenous requests for objects are routed towards nodes that store them; as a result, object traffic in the network is determined not only by demand but, crucially, by where objects are cached. We determine how to place objects in caches to attain a certain design objective, such as, e.g., minimizing network congestion or retrieval delays. We show that for a broad class of objectives, including minimizing both the expected network delay and the sum of network queue lengths, this optimization problem can be cast as an NP- hard submodular maximization problem. We show that so-called continuous greedy algorithm attains a ratio arbitrarily close to $1 - 1/e \approx 0.63$ using a deterministic estimation via a power series; this drastically reduces execution time over prior art, which resorts to sampling. Finally, we show that our results generalize, beyond M/M/1 queues, to networks of M/M/k and symmetric M/D/1 queues.

==> Kelly Cache Networks/beyond.tex <==
As discussed in Section~\ref{sec:model}, the classes of M/M/1 queues for which the supermodularity of the cost functions arises is quite broad, and includes FIFO, LIFO, and processor sharing queues. In this section, we discuss how our results extend to even broader families of queuing networks.  %All proofs can be found in \techrep{the appendix}{\cite{techrep}}. %Specifically, our results extend to general networks of queues that have a product form steady-state distribution, under which the objective is to minimize a supermodular cost function.
		\techrep{Chapter 3 of Kelly~\cite{kelly} provides a general framework for a set of queues for which service times are exponentially distributed; for completeness, we also summarize this  in Appendix~\ref{app:kelly}. %Differing from Section~\ref{sec:model}, service rates $\mu_e$ in this model are allowed to depend on network state. %Kelly shows that this class of queues indeed have a product form distribution. Please refer to Appendix \ref{app:kelly} for the definition of the queues and their steady-state distribution.
		%Examples of such queues includes M/M/1, M/M/k, M/M/m/k. 
		A large class of networks can be modeled by this framework, including networks of M/M/$k$ queues; all such networks maintain the property that steady-state distributions have a product form.  
This allows us to}{We first} extend our results to M/M/$k$ queues for two cost functions $C_e$: %As in the case of M/M/1 networks, the first is the expected number of packets in a queue. The second is the \emph{probability of queuing}, i.e., the probability that an arriving packet encounters all $k$ servers to be busy (given by the so-called Erlang C formula \cite{datanetworks}). Our results readily extend to both of these cases: %One objective function which is known as Erlang C formula \cite{datanetworks}, measures the probability that an arriving packet will find all $k$ servers in the queue busy, and hence, is forced to wait in the queue. The other function computes the expected number of packets waiting for or under transmission in the queue.
		\begin{lemma}\label{lemma:mmk}
			For a network of M/M/k queues, both the  queuing probability\footnote{This is %the probability that an arriving packet finds all $k$ servers to be busy (
			given by the so-called Erlang C formula \cite{datanetworks}.} and the expected queue size are non-increasing and supermodular over sets $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$.
		\end{lemma}
		%\begin{proof}
	        %The proof can be found  in \techrep{Appendix \ref{app:mmk}.}{\cite{techrep}.} 
We note that, as an immediate consequence of Lemma~\ref{lemma:mmk} and Little's theorem, both the sum of the expected delays per queue, but also the expected delay of an arriving packet, are also  supermodular and non-decreasing.
		%\end{proof}
		
		Product-form  steady-state distributions arise also in settings where service times are not exponentially distributed. A large class  of quasi-reversible queues, named {\em symmetric queues} exhibit this property (c.f.~Section 3.3 of \cite{kelly} and Chapter 10 of \cite{nelson}). \techrep{For completeness, we again summarize symmetric queues in Appendix \ref{app:symmetric}.}{}		%A large set of queues can be modeled as symmetric queues. For instance, it can be shown that Last-In First-Out (LIFO) with preemptive resume,  queues with shared processors, and finite-capacity queues can all be modeled as symmetric queues.  An interesting example of queues with general packet scheduling distribution is one deterministic service effort, since transmission time of packets with equal size, being approximately proportional to their size, is deterministic. 
In the following lemma %, whose proof is in \techrep{Appendix~\ref{app:proof-symmetric}}{\cite{\techrep}},
 we leverage the product form of symmetric queues to extend our results to M/D/1 symmetric queues \cite{datanetworks}.
		\begin{lemma}\label{lemma:symmetric}
			For a network of M/D/1 symmetric queues, the expected queue size is non-increasing and supermodular over sets $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$.
		\end{lemma}
		%		\begin{proof}
		%			Please see Appendix \ref{app:proof-symmetric}.
		%		\end{proof}
		Again, Lemma~\ref{lemma:symmetric} and Little's theorem imply that this property also extends to network delays.
		It is worth noting that conclusions similar to these in Lemmas \ref{lemma:mmk} and \ref{lemma:symmetric} are not possible for all general queues with product form distributions. In particular, also we prove the following negative result: %  for $M/M/1/k$ queues: %one cannot find a monotone function which is monotone and supermodular over sets  sets $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$.
		%$\rho_{u,v}(\mathbf{x})$ is generally non-monotone and neither submodular, nor supermodular.
		\begin{lemma} There exists a network of  M/M/1/k queues, containing a queue $e$, for which no strictly monotone function $C_e$ of the load $\rho_e$ at a queue $e$ is non-increasing and supermodular over sets $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$. In particular, the expected  size of queue $e$ is neither monotone nor supermodular. 
			\label{lemma:example}
		\end{lemma}
			%The proof can be found in Appendix \ref{app:md1}. 
	
%		One conclusion of Lemma \ref{lemma:example} is that the expected number of packets in an arbitrary network of M/M/1/k queues is non-increasing and supermodular over sets $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$, since the expected number of packets in a queue is strictly monotone in the queue's traffic load.


==> Kelly Cache Networks/conclusions.tex <==
Our analysis suggests feasible object placements targeting many design objectives of interest, including system size  and delay, can be determined using combinatorial techniques. Our work leaves the exact characterization of approximable objectives for certain classes of queues, including M/M/1/k queues, open. %; providing guarantees for M/M/1/k queues, that are not amenable to an analysis via submodular maximization, is also an important open problem.
Our work also leaves open problems relating to stability. This includes the characterization of the stability region of arrival rates $\Lambda = \cup_{\mathbf{x}\in \domain} \Lambda(\mathbf{x})$.  It is not clear whether determining membership in this set (or, equivalently, given $\lambda$, determining whether  there exists a $\mathbf{x}\in \domain$ under which the system is stable) is NP-hard or not, and whether this region can be somehow approximated. Finally, all algorithms presented in this paper are offline: identifying how to determine placements in an online, distributed fashion, in a manner that attains a design objective (as in \cite{ioannidis2016adaptive,ioannidis2017jointly}), or even stabilizes the system (as in \cite{yeh2014vip}), remains an important open problem.


==> Kelly Cache Networks/experiments.tex <==
\begin{table}[!t]
\caption{Graph Topologies and Experiment Parameters.}\label{tab:networks}
\begin{scriptsize}
\begin{tabular}{  p{13mm} p{3mm} p{3mm} p{3mm} p{2mm} p{2mm} p{2.5mm} cc}%p{7mm}p{7mm}} 
Graph & $|V|$ & $|E|$ & $|\catalog|$ & $|\demand|$ &  $|Q|$ & $c_v$ & $F_{\text{PL}}\!(\mathbf{x}_{\text{RND}})$ & $F_{\text{UNI}}\!(\mathbf{x}_{\text{RND}})$\\
\hline
 \texttt{ER} &100 & 1042  & 300 & 1K & 4 & 3& 2.75& 2.98\\
 \texttt{ER-20Q} &100 & 1042  & 300 & 1K & 20 & 3& 3.1& 2.88\\
\texttt{HC}&128 & 896  & 300 & 1K & 4 & 3& 2.25 & 5.23\\
\texttt{HC-20Q}&128 & 896  & 300 & 1K & 20 & 3& 2.52 & 5.99\\
 \texttt{star} & 100 & 198 & 300 & 1K & 4 & 3 & 6.08 & 8.3\\
 \texttt{path} & 4 & 3 & 2 & 2 &1 &1& 1.2 &1.2\\
 \texttt{dtelekom} & 68 & 546 & 300 & 1K & 4 & 3 &2.57 &3.66\\
  \texttt{abilene} & 11 & 28 & 4 &2& 2& 1/2 & 4.39 &4.39\\
  \texttt{geant} &22 & 66& 10&100 & 4& 2 &19.68&17.22
\end{tabular}
\end{scriptsize}
\end{table}
\begin{figure}[!t]
\vspace{-4mm}
\centering 
    \includegraphics[width=0.8\columnwidth]{abilene_concocted_graph.pdf}
    \caption{The \texttt{abilene} topology. We consider a catalog size of $|\catalog|=4$ and 4 requests $(|\demand|=4)$. Requests originate from $|Q|=2$ nodes, $b$ and $i$. Three edges have a high service rate $M\gg 1$, and the rest have a low service rate $2+ \varepsilon$. Only nodes $a, g,$ and $h$ can cache items, and have capacities  2, 1, and 1, respectively. We set $M=200$ and $\varepsilon=0.05$ in our experiments. Greedy is  0.5-approximate in this instance.}\label{fig:halfistight2}
\end{figure}
\noindent\textbf{Networks.} We execute Algorithms~\ref{alg:greedy}~and~\ref{alg:cg} over 9 network topologies, summarized in Table~\ref{tab:networks}. 
%Graph \texttt{balanced-tree} is a complete binary tree of 123 nodes. 
Graphs \texttt{ER} and \texttt{ER-20Q} are the same 100-node Erd\H{o}s-R\'enyi graph with parameter $p=0.1$. Graphs \texttt{HC} and \texttt{HC-20Q} are the same hypercube graph with 128 nodes, and graph \texttt{star} is a star graph with 100 nodes. The graph \texttt{path} is the topology shown in Fig.~\ref{fig:halfistight}. 
The last 3 topologies, namely, \texttt{dtelekom}, \texttt{geant}, and \texttt{abilene} represent the Deutsche Telekom, GEANT, and Abilene backbone networks, %\cite{rossi2011caching},
respectively. The latter is also shown in Fig.~\ref{fig:halfistight2}. 


\begin{figure}[!t]
\vspace{-3mm}
	\centering
	\subfloat[Power-law demand]{
		\includegraphics[width=\columnwidth]{problem_1000demands_300catalog_size_mincap_3maxcap_3_100_powerlaw.pdf}\label{cache_gain_plaw}
	}
	\vspace{-4mm}
	
	\subfloat[Uniform demand]{
		\includegraphics[width=\columnwidth]{problem_1000demands_300catalog_size_mincap_3maxcap_3_100_uniform.pdf}\label{cache_gain_uniform}
	}
\caption{Caching gains for different topologies and different arrival distributions, normalized by the gains corresponding to RND, reported in Table.~\ref{tab:networks}. Greedy performs comparatively well. However, it attains sub-optimal solutions for \texttt{path} and \texttt{abilene}; these solutions are worse than RND. CG-RS500 has a poor performance compared to other variations of the continuous-greedy algorithm.}\label{cache_gain_1}
\end{figure}
\begin{figure}[!t]\vspace{-4mm}
    \includegraphics[width=\columnwidth]{time_1000demands_300catalog_size_mincap_3maxcap_3_100_powerlaw.pdf}
    \caption{Running time for different topologies and power-law arrival distribution, in seconds. CG-RS500 is slower than power series estimation CG-PS1 and CGT, sometimes exceeding CG-PS2 as well.}\label{fig:time}
    \vspace{-2mm}
\end{figure}


\begin{figure}[!t]
\vspace{-4mm}
\centering

     \subfloat[\texttt{abilene}]{\includegraphics[width=0.5\columnwidth]{dvrs_abilene_1000demands_300catalog_size_mincap_3maxcap_3_100_powerlaw.pdf}}
     \subfloat[\texttt{path}]{\includegraphics[width=0.5\columnwidth]{dvrs_special_case_1000demands_300catalog_size_mincap_3maxcap_3_100_powerlaw.pdf}}
     
\caption{Caching gain vs. $M$. As the discrepancy between the service rate of low-bandwidth and high-bandwidth links increases, the performance of Greedy deteriorates.}\label{fig:M}
\end{figure}



\noindent\textbf{Experimental Setup.} 
For  \texttt{path} and \texttt{abilene}, we set demands, storage capacities, and service rates as illustrated in Figures~\ref{fig:halfistight} and \ref{fig:halfistight2}, respectively. Both of these settings induce an approximation ratio close to $1/2$ for greedy. 
For all remaining topologies,  we consider a catalog of size $|\catalog|$ objects; for each object, we select 1 node  uniformly at random (u.a.r.) from $V$ to serve as the designated server for this object. To induce traffic overlaps, we also select $|Q|$ nodes u.a.r.~that serve as sources for requests; all requests originate from these sources. 
All caches are set to the same storage capacity, i.e., $c_v=c$ for all $v\in V$. 
 We generate a set of $|\demand|$ possible  types of requests. For each request type $r\in \demand$, $\lambda^r=1$ request per second, and   path $p^r$ is generated by selecting a source among the $|Q|$ sources u.a.r., and routing towards the designated server of object $i^r$ using a shortest path algorithm. We consider two ways of selecting objects $i^r\in \catalog$:   in the \emph{uniform} regime, $i^r$ is selected u.a.r. from the catalog $\catalog$;  in the \emph{power-law} regime, $i^r$ is selected from the catalog $\catalog$ via a power law distribution with exponent $1.2$. All  the parameter values, e.g., catalog size $|\catalog|$, number of requests $|\demand|$, number of query sources $|Q|$, and caching capacities $c_v$ are presented in Table~\ref{tab:networks}. 

We construct heterogeneous service rates as follows. Every queue service rate is either set to a low value $\mu_e=\mu_{\text{low}}$ or a high value $\mu_e=\mu_{\text{high}},$ for all $e \in E.$ We select $\mu_{\text{low}}$ and $\mu_{\text{high}}$ as follows.  Given the demands $r\in \demand$ and the corresponding arrival rates $\lambda^r$, we compute the highest load under no caching ($\mathbf{x}=\mathbf{0}$), i.e., we find  
$\lambda_{\max} = \max_{e\in E} \sum_{r:e\in p^r} \lambda^r.$
We then set $\mu_{\text{low}} = \lambda_{\max}\times 1.05$ and $\mu_{\text{high}} = \lambda_{\max}\times 200$. We  set the service rate to $\mu_{\text{low}}$ for all congested edges, i.e., edges $e$ s.t.~ $\lambda_e=\lambda_{\max}$. We set the service rate for each remaining edge $e\in E$ to $\mu_{\text{low}}$ independently with probability 0.7, and to $\mu_{\text{high}}$ otherwise.  Note that, as a result $\textbf{0}\in \domain_{\bm{\lambda}}=\domain$, i.e., the system is stable even in the absence of caching and, on average, 30 percent of the edges have a high service rate. 


\begin{figure}[!t]
\vspace{-1mm}
\centering 
     \subfloat[\texttt{dtelekom}]{\includegraphics[width=0.5\columnwidth]{dtelekom_rates_1000demands_300catalog_size_mincap_3maxcap_3_powerlaw.pdf}}
     \subfloat[\texttt{ER}]{\includegraphics[width=0.5\columnwidth]{erdos_renyi_rates_1000demands_300catalog_size_mincap_3maxcap_3_powerlaw.pdf}}
\caption{Caching gain vs. arrival rate. As the arrival rate increases caching gains get larger.}\label{fig:rates}
\vspace{-1mm}
\end{figure}


\begin{figure}[!t]
\vspace{-1mm}
\centering
     \subfloat[\texttt{dtelekom}]{\includegraphics[width=0.5\columnwidth]{dtelekom_capacities_1000demands_300catalog_size_mincap_3maxcap_3_powerlaw.pdf}}
     \subfloat[\texttt{ER}]{\includegraphics[width=0.5\columnwidth]{erdos_renyi_capacities_1000demands_300catalog_size_mincap_3maxcap_3_powerlaw.pdf}}
     \caption{Caching gain vs. cache capacity. As caching capacities increase, caching gains rise. }\label{fig:cap}
\end{figure}


\noindent\textbf{Placement Algorithms.} We implement several placement algorithms: (a) \emph{Greedy}, i.e., the greedy algorithm (Alg.~\ref{alg:greedy}), (b) \emph{Continuous-Greedy with Random Sampling} (CG-RS), i.e., Algorithm~\ref{alg:cg} with a gradient estimator based on sampling, as described in Sec.~\ref{sec:sample}, (c) \emph{Continuous-Greedy with Taylor approximation} (CGT), i.e.,    Algorithm~\ref{alg:cg} with a gradient estimator based on the Taylor expansion, as described in Sec.~\ref{sec:taylor}, and (d) \emph{Continuous-Greedy with Power Series approximation} (CG-PS), i.e., Algorithm~\ref{alg:cg} with a gradient estimator based on the power series expansion, described also in Sec.~\ref{sec:taylor}. In the case of CG-RS, we collect 500 samples, i.e., $T=500$. In the case of CG-PS we tried the first and second order expansions of the power series as CG-PS1 and CG-PS2, respectively. In the case of CGT, we tried the first-order expansion $(L=1)$. In both cases, subsequent to the execution of Alg.~\ref{alg:cg} we produce an integral solution in $\domain$ by rounding via the swap rounding method \cite{chekuri2010dependent}. All continuous-greedy algorithms use $\gamma=0.001.$ We also implement a random selection algorithm (RND), which caches $c_v$ items at each node $v \in V$, selected uniformly at random. We repeat RND 10 times, and report the average running time and caching gain. 

\noindent\textbf{Caching Gain Across Different Topologies.} 
The caching gain $F(\mathbf{x})$ for $\mathbf{x}$ generated by different placement algorithms, is shown for power-law arrival distribution and uniform arrival distribution in Figures ~\ref{cache_gain_plaw} and \ref{cache_gain_uniform}, respectively. The values are normalized by the gains obtained by RND, reported in Table~\ref{tab:networks}. Also, the running times of the algorithms for power-law arrival distribution are reported in Fig.~\ref{fig:time}.
As we see in Fig.~\ref{cache_gain_1}, Greedy is comparable to other algorithms in most topologies. However, for topologies \texttt{path} and \texttt{abilene} Greedy obtains a sub-optimal solution, in comparison to the continuous-greedy algorithm. In fact, for \texttt{path} and \texttt{abilene} Greedy performs even worse than RND. 
In Fig.~\ref{cache_gain_1}, we see that the continuous-greedy algorithms with gradient estimators based on Taylor and Power series expansion, i.e., CG-PS1, CG-PS2, and CGT outperform CG-RS500 in most topologies. Also, from Fig.~\ref{fig:time}, we see that CG-RS500 runs 100 times slower than the continuous-greedy algorithms with first-order gradient estimators, i.e., CG-PS1 and CGT. Note that 500 samples are significantly below the value\techrep{, stated in Theorem~\ref{thrm:sampling},}{} needed to attain the theoretical guarantees of the continuous-greedy algorithm, which is quadratic in $|V||\catalog|$. 


\noindent\textbf{Varying Service Rates.}
For topologies \texttt{path} and \texttt{abilene}, the approximation ratio of Greedy is $\approx 0.5.$ This ratio  is a function of service rate of the high-bandwidth link $M.$  In this experiment, we explore the effect of varying $M$ on the performance of the algorithms in more detail. We plot the caching gain obtained by different algorithms for \texttt{path} and \texttt{abilene} topologies, using different values of $M\in \{M_{\min},10,20,200\},$ where $M_{\min}$ is the value that puts the system on the brink of instability, i.e., 1 and $2+\epsilon$ for \texttt{path} and \texttt{abilene}, respectively. Thus, we gradually increase the discrepancy between the service rate of low-bandwidth and high-bandwidth links. 
The corresponding caching gains are plotted in Fig.~\ref{fig:M}, as a function of $M$. We see that as $M$ increases the gain attained by Greedy worsens in both topologies: when $M=M_{\min}$ Greedy matches the performance of the continuous-greedy algorithms, in both cases. However, for higher values of $M$ it is beaten not only by all variations of the continuous-greedy algorithm, but by RND as well. 


\noindent\textbf{Effect of Congestion on Caching Gain.}
In this experiment, we study the effect of varying arrival rates $\lambda^r$ on caching gain $F$. We report results only for the \texttt{dtelekom} and \texttt{ER} topologies and power-law arrival distribution. We obtain the cache placements $\mathbf{x}$  using the parameters presented in Table~\ref{tab:networks} and different arrival rates: $\lambda^r\in\{0.65, 0.72, 0.81, 0.9, 1.0\},$ for $r \in \demand$. Fig.~\ref{fig:rates} shows the caching gain attained by the placement algorithms as a function of arrival rates. We observe that as we increase the arrival rates, the caching gain attained by almost all algorithms, except RND, increases significantly. Moreover, CG-PS1, CG-PS2, CGT, and Greedy have a similar performance, while CG-RS500 achieves lower caching gains. 

\noindent\textbf{Varying Caching Capacity.}
In this experiment, we study the effect of increasing cache capacity $c_v$ on the acquired caching gains. Again, we report the results only for the \texttt{dtelekom} and \texttt{ER} topologies and power-law arrival distribution. We evaluate the caching gain obtained by different placement algorithms using the parameters of Table~\ref{tab:networks} and different caching capacities: $c_v\in\{1,3, 10,30\}$ for $v \in V.$ The  caching gain is plotted in Fig.~\ref{fig:cap}. As we see, in all cases the obtained gain increases, as we increase the caching capacities. This is expected: caching more items  reduces traffic and delay,  increasing the gain. 



==> Kelly Cache Networks/greedy.tex <==
Constraints \eqref{eq:fcon} define a (partition) matroid \cite{calinescu2011,femtocaching}. This, along with the submodularity and monotonicity of $F$ imply that we can produce a solution  within $\frac{1}{2}$-approximation from the optimal via the \emph{greedy} algorithm \cite{greedy}. The algorithm, summarized in Alg.~\ref{alg:greedy}, iteratively allocates items to caches that yield the largest marginal gain.
\begin{comment}
proceeds iteratively as follows. Starting from the initial feasible content placement $\mathbf{x}_0$, the greedy algorithm  adds a single object to a cache at each iteration, i.e., sets $x_{v^*i^*}=1$ for some $v^*\in V$, $i^*\in \catalog$.  If $\mathbf{x}$ is the present solution at the beginning of an iteration, the cache-item pair $(v^*,i^*)$ is selected as follows: 
\begin{equation}
(v^*,i^*)=\mathop{\arg \max}_{(v,i) \in A(\mathbf{x})} \left( F(\mathbf{x}+\mathbf{e}_{vi}) -F(\mathbf{x}) \right)
%F_{\mathbf{x}}((v',i')),
\end{equation}
where $A(\mathbf{x}):= \{(v,i)\in V\times \catalog: \mathbf{x}+\mathbf{e}_{vi} \in \domain \}$, and  $\mathbf{e}_{vi}\in\{0,1\}^{|V||\catalog|}$ is a unit vector with its $(v,i)$-th element equal to one and the remaining elements equal to zero.
%\begin{equation}
%F_{\mathbf{x}}((v,i)) :=  F(\mathbf{x}+\mathbf{e}_{vi}) -F(\mathbf{x}), \text{ for } (v,i) \in A(\mathbf{x}),
%\end{equation}
%and $\mathbf{e}_{vi}$ is a unit vector with $(v,i)$-th element equals to one and the rest equal to zero. 
This procedure continues until $A(\mathbf{x}) =\emptyset$.  
\end{comment}
The solution produced by Algorithm \ref{alg:greedy}  is guaranteed  to be  within a $\frac{1}{2}$-approximation ratio of the optimal solution of \textsc{MaxCG} \cite{greedy2}.  The approximation guarantee of $\frac{1}{2}$ is tight: %; we prove this below.
\begin{lemma}\label{lem:tight} For any $\varepsilon>0$, there exists a cache network  the greedy algorithm solution is within $\frac{1}{2}+\varepsilon$ from the optimal, when the objective is the sum of expected delays per edge.
\end{lemma}
\begin{comment}
\begin{proof}
Consider the path topology illustrated in Fig.~\ref{fig:halfistight}. Assume that requests for files 1 and 2 are generated at node $u$ with rates $\lambda_1=\lambda_2=\delta$, for some  $\delta\in(0,1)$. Files 1 and 2 are stored permanently at $v$ and $z$, respectively. Caches exist only on $u$ and $w$, and have capacity $c_u=c_w=1$. Edges $(u,v)$, $(w,z)$ have bandwidth $\mu_{(u,v)}=\mu_{(w,z)}=1$, while edge $(u,w)$ is a high bandwidth link, having capacity $M\gg 1$. Let $\mathbf{x}_0=\mathbf{0}$.
The greedy algorithm starts from empty caches  and adds item 2 at cache $u$. This is because the caching gain from this placement is $c_{(u,w)}+c_{(w,z)}= \frac{1}{M-\delta} + \frac{1}{1-\delta}$, while the caching gain of all other decisions is at most $\frac{1}{1-\delta}$. Any subsequent caching decisions do not change the caching gain. The optimal solution is to cache item 1 at $u$ and item 2 at $w$, yielding a caching gain of $2/(1-\delta)$. Hence, the greedy solution attains an approximation ratio 
%$$\frac{ \frac{1}{M-\delta} + \frac{1}{1-\delta}   }{\frac{2}{1-\delta}} =
$0.5\cdot (1+\frac{1-\delta}{M-\delta}).$
By  appropriately choosing $M$ and $\delta$, this can be made arbitrarily close to 0.5. 
\end{proof}
\end{comment}
\techrep{The proof of Lemma~\ref{lem:tight} can be found in Appendix \ref{app:proofoflem:tight}.}{} The instance under which the bound is tight is given in Fig.~\ref{fig:halfistight}\techrep{}{ (see also \cite{techrep})}.
%We note that it is easy to extend Lemma~\ref{lem:tight} to other objectives, including, e.g., expected delay, queue size, etc. We note also that tight instances can be constructed using caches with capacities larger than 1 (see, e.g., Fig.~\ref{fig:halfistight2}). 
As we discuss in Sec.~\ref{sec:experiments}, the greedy algorithm performs well in practice for some topologies; however, Lemma~\ref{lem:tight} motivates us to seek alternative algorithms, that attain  improved approximation guarantees. %over greedy.

\begin{figure}[!t]
\centering 
    \includegraphics[width=0.8\columnwidth]{counter_example.pdf}
    \caption{A path graph, illustrating that the $1/2$-approximation ratio of greedy is tight. Greedy caches item $2$ in node $u$, while the optimal decision is to cache item $1$ in $u$ and item $2$ in node $w$. For $M$ large enough, the approximation ratio can be made arbitrarily close to 1/2.  In our experiments in Sec.~\ref{sec:experiments}, we set $\delta=0.5$ and $M=200$.}\label{fig:halfistight}
\end{figure}

  \algsetup{linenosize=\scriptsize} 
\begin{algorithm}[!t]
		\caption{Greedy}\label{alg:greedy}
\begin{scriptsize}
		\begin{algorithmic}[1]
			\REQUIRE $F:\domain \rightarrow \reals_+,\mathbf{x}_0$
			\STATE   $\mathbf{x}\leftarrow \mathbf{x}_0$
			\WHILE{ $A(\mathbf{x}):= \{(v,i)\in V\times \catalog: \mathbf{x}+\mathbf{e}_{vi} \in \domain \}$  is not empty }
			\STATE  $(v^*,i^*) \leftarrow \mathop{\arg \max}_{(v,i) \in A(\mathbf{x})} \left( F(\mathbf{x}+\mathbf{e}_{vi}) -F(\mathbf{x}) \right)$ \label{line: max} 
			\STATE $\mathbf{x} \leftarrow \mathbf{x}+\mathbf{e}_{v^*i^*}$
			\ENDWHILE
			\RETURN $\mathbf{x}\;$
		\end{algorithmic}
\end{scriptsize}
	\end{algorithm}




==> Kelly Cache Networks/intro.tex <==
Kelly networks \cite{kelly} are multi-class networks of queues capturing a broad array of queue service disciplines, including FIFO, LIFO, and processor sharing. Both Kelly networks and their  generalizations (including networks of quasi-reversible and symmetric queues) are well studied and classic topics \cite{kelly,gallager-stochastic,nelson,chen2013fundamentals}. One of their most appealing properties is that their steady-state distributions have a product-form: as a result, steady state properties such as expected queue sizes, packet delays,  and server occupancy rates have closed-form formulas 
  as functions of, e.g., routing and scheduling policies.

In this paper, we  consider Kelly networks in which nodes are equipped with caches, i.e., storage devices of finite capacity, which can be used to store objects. Exogenous  requests for objects  are routed towards nodes that store them; upon reaching a node that stores the requested object, a response packet containing the object is routed towards the request source. As a result, object traffic in the network is determined not only by the demand but, crucially, by where objects are cached.
This abstract setting is motivated by--and can be used to model--various networking applications involving the placement and transmission of content. This includes information centric networks ~\cite{jacobson2009networking,yeh2014vip,ioannidis2016adaptive}, content delivery networks~\cite{borst2010distributed,dehghan2014complexity}, web-caches~\cite{laoutaris2004meta,che2002hierarchical,zhou2004second},  wireless/femtocell networks \cite{shanmugam2013femtocaching,naveen2015interaction,poularakis2013approximation}, and 
 peer-to-peer networks~\cite{lv2002search,cohen2002replication}, to name a few.

In many of these applications, determining the \emph{object placement}, i.e., how to place objects in network caches, is a decision that can be made by the network designer in response to object popularity and demand. To that end, we are interested in determining how to place objects in caches so that  traffic attains a design objective such as, e.g., minimizing delay.

We make the following contributions.
%\begin{itemize}
%\item We \emph{introduce Kelly cache networks}, namely, multi-class networks of queues in which nodes are equipped with caches capable of storing objects.
%\item
First, we study the problem of optimizing the placement of objects in caches in  Kelly cache networks of M/M/1 queues, with the objective of minimizing a cost function of the system state. We show that, for a broad class of cost functions, including packet delay, system size, and server occupancy rate, \emph{this optimization amounts to a submodular maximization problem with matroid constraints}. This result applies to general Kelly networks with fixed service rates; in particular, it holds for FIFO, LIFO, and processor sharing  disciplines at each queue.
%\item We leverage this connection to submodular optimization to study approximation algorithms for the resulting (NP-hard) problems. It is known that the classic greedy algorithm \cite{greedy} produces a solution with a 0.5 approximation ratio, while the so-called continuous-greedy algorithm~\cite{calinescu2011} yields a ratio of $1-1/e\approx 0.63$. We prove that  \emph{the  0.5-approximation ratio of the greedy algorithm is tight}, %This 
%motivating  our  study of the continuous-greedy algorithm.
%\item 

The so-called continuous greedy algorithm \cite{calinescu2011} attains a $1-1/e$ approximation for this NP-hard problem. However, it does so by computing an expectation over a random variable with exponential support  via randomized sampling. The number of samples required to attain the $1-1/e$ approximation guarantee can be prohibitively large in realistic settings. Our second contribution is to show that, for Kelly networks of M/M/1 queues, \emph{this randomization can be entirely avoided}: a closed-form solution can be computed using the Taylor expansion of our problem's objective. To the best of our knowledge, we are the first to identify a submodular maximization problem that exhibits this structure, and to exploit it to eschew sampling.
%
%item
Finally, we extend our results to \emph{networks of M/M/$k$  and symmetric M/D/1  queues}, and %, showing that optimizing quantities such as expected queue lengths and the probability of encountering a busy server can again be cast as submodular maximization problems. 
prove  a negative result: submodularity does \emph{not} arise in networks of M/M/1/$k$ queues.
 We extensively evaluate our proposed algorithms over several synthetic and real-life topologies. % of Kelly cache networks.  
%\end{itemize}

The remainder of our paper is organized as follows. We review related work in Sec.~\ref{sec:related}. We present our mathematical model of a Kelly cache network in Sec.~\ref{sec:model}, and our results on submodularity and the continuous-greedy algorithm in networks of M/M/1 queues in Sections~\ref{sec:subm} and~\ref{sec:contgreed}, respectively. Our extensions are described in Sec.~\ref{sec:beyond}; our numerical evaluation is in Sec.~\ref{sec:experiments}. Finally, we conclude in Sec.~\ref{sec:conclusions}. \techrep{}{For brevity, we omit detailed proofs, which can be found in \cite{techrep}.}


==> Kelly Cache Networks/main_res.tex <==
\section{Submodularity and the Greedy Algorithm}\label{sec:subm}
Problem \textsc{MinCost} is NP-hard; this is true even when cost functions $c_e$ are linear, and the objective is to minimize the sum of the loads per edge \cite{ioannidis2016adaptive,femtocaching}. In what follows, we outline our methodology for solving this problem; it relies on the fact that the objective of \textsc{MinCost} is a \emph{supermodular set function}; our first main contribution is to show that this property is a direct consequence of Assumption~\ref{as:conv}. 

%The presence of submodularity allows us to cast  \textsc{MinCost} into a submodular maximization problem subject to matroid constraints. An algorithm that attains a $1-1/e$ approximation from the optimal exists for this general setting (i.e., for arbitrary submodular functions and matroid constraints) \cite{calinescu2011}; this algorithm relies on estimating the gradient of the objective via random sampling. Our second main contribution is to show that the objective of \textsc{MinCost} exhibits additional structure, which we  exploit to eschew randomization altogether: indeed, we show that a biased estimator of the gradient can be computed in polynomial time via the Taylor approximation of the objective.

%\section{Optimization}
%\subsection
\noindent\textbf{Cost Supermodularity and Caching Gain.}
%Our first main result establishes an important property of the objective function of \textsc{MinCost}. 
 First, observe that the cost function $C$ in \textsc{MinCost} can be naturally  expressed as a set function. Indeed, for $S\subset V\times \catalog$, let $\mathbf{x}_S\in \{0,1\}^{|V| |\catalog|} $ be the binary vector whose support  is $S$ (i.e., its non-zero elements are indexed by $S$). As there is a 1-1 correspondence between a binary vector $\mathbf{x}$ and its support $\supp(\mathbf{x})$,  we can interpret $C:\{0,1\}^{|V| |\catalog|}\to \reals_+$ as  set function $C:V\times \catalog:\to\reals_+$ via
$C(S)\triangleq C(\mathbf{x}_S).$ Then, the following theorem holds:
\begin{comment}
\begin{theorem}\label{thm:coststruct}
Under Assumption~\ref{as:conv}, function $C: \{0,1\}^{|V|\times |\catalog|}$ is non-increasing, i.e.
$$C(X)\geq C(X') \text{ for all } X\leq X',$$
as well as \emph{supermodular}, i.e.,
for all $X,X'\in \domain_\lambda$ s.t.~$X\geq X'$, and all $u\in V$,  $i\in \catalog$,
$$C(X+E_{ui}) -C(X) \leq C(X'+e_{ui}) -C(X') $$
where $E_{ui}\in \{0,1\}^{|V|\times |\catalog|}$ is a binary matrix whose only non-zero coordinate is at row $v$ and column $i$.
\end{theorem}
\end{comment}
\begin{theorem}\label{thm:coststruct}
Under Assumption~\ref{as:conv},  
$C(S)\triangleq C(\mathbf{x}_S)$
 is non-increasing and supermodular  over  $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$.
\end{theorem}
\techrep{A detailed proof of Theorem~\ref{thm:coststruct} can be found in Appendix~\ref{app:coststruct}.}
{\begin{proof}[Proof (Sketch)]
It is easy to verify that $\rho_{e}(S), \forall e\in E$, is supermodular and non-increasing in $S$. By Assumption \ref{as:conv} $C_e$ is a non-decreasing function, so $C_e(S)\triangleq C_{e}(\rho_{e}(S))$ is non-increasing. The theorem then follows from Assumption \ref{as:conv} and the fact that if $f:\reals\to\reals$ is  convex and non-decreasing and $g: \mathcal{X}\to \reals$ is  non-increasing supermodular then $h(\mathbf{x})\triangleq f(g(\mathbf{x}))$ is also supermodular.\end{proof}}
%
 In light of the observations in Sec.~\ref{sec:mincost} regarding Assumption~\ref{as:conv},  Thm.~\ref{thm:coststruct} implies that supermodularity arises \emph{for a broad array of natural cost objectives}, including expected delay and system size; it also applies under the \emph{full generality of Kelly networks}, including FIFO, LIFO, and round robin service disciplines.
Armed with this theorem, we turn our attention to converting \textsc{MinCost} to a \emph{submodular maximization} problem. In doing so, we face the problem that domain $\domain_{\bm{\lambda}}$, determined not only by storage capacity constraints, but also by stability, may be difficult to characterize. Nevertheless, we show that a problem that is amenable to approximation can be constructed, provided that a placement $\mathbf{x}_0 \in \domain_{\bm{\lambda}}$ is known.


%	As shown in Shanmugam et al. \cite{femtocaching}, problem \eqref{opt:mincost} is NP-hard. However, we show in the following that $C(X)$ is a supermodular and non-increasing function. In addition, it can be shown that $\mathcal{D}_1$ is a (partition) matroid \cite{femtocaching}. Hence, we can use combinatorial optimization techniques to reach a constant approximation solution with some optimality guarantee using a greedy algorithm.
	
In particular, suppose that we have access to a single $\mathbf{x}_0\in \domain_{\bm{\lambda}}$. We define the \emph{caching gain} $F: \domain_{\bm{\lambda}} \to \reals_+$ as $F(\mathbf{x}) = C(\mathbf{x}_0)- C(\mathbf{x}). $
Note that, for $\mathbf{x}\geq \mathbf{x}_0$, $F(\mathbf{x})$ is the relative decrease in the cost compared to the cost under $\mathbf{x}_0$. We consider the following optimization problem:\\
	\begin{subequations}\label{opt:maxcg}
{\hspace*{\stretch{1}} \textsc{MaxCG} \hspace*{\stretch{1}} }\vspace{-0.8em}
		\begin{align}
			\text{Maximize:}&\quad F(\mathbf{x}) = C(\mathbf{x}_0) - C(\mathbf{x})\label{eq:fobj}\\   
			\text{subj.~to:}&\quad \mathbf{x} \in\domain, \mathbf{x}\geq \mathbf{x}_0 \label{eq:fcon}
	        \end{align} 
	\end{subequations}
Observe that, if $\mathbf{0}\in \domain_{\bm{\lambda}}$, then $\domain_{\bm{\lambda}} =\domain$; in this case, taking $\mathbf{x}_0=\mathbf{0}$ ensures that problems \textsc{MinCost} and \text{MaxCG} are equivalent. If $\mathbf{x}_0\neq \textbf{0}$, the above formulation attempts to maximize the gain restricted to placements $\mathbf{x}\in \domain$ that dominate $\mathbf{x}_0$: such placements necessarily satisfy $\mathbf{x}\in \domain_{\bm{\lambda}}$. 
Thm.~\ref{thm:coststruct} has the following immediate implication: 
\begin{cor}The caching gain $F(S)\triangleq F(\mathbf{x}_S)$ is non-decreasing and submodular  over  $\{\supp(\mathbf{x}): \mathbf{x}\in \domain_{\bm{\lambda}}\}$.
\end{cor}	
%Hence, Thm.~\ref{thm:coststruct} implies that \eqref{opt:maxcg} involves a positive, non-decreasing submodular objective. As such, there exist polynomial time approximation algorithms for its solution; we list two below.

\noindent\textbf{Greedy Algorithm.}\label{sect:greedy}
\input{greedy}

%	\subsection{Problem Transformation: Submodular Maximization Problem}
%	\label{sec:transformation}
%	As shown in previous section, $C(X)$ is a non-increasing supermodular function. Since minimizing a supermodular function is often more complicated than maximizing a submodular function \cite{Mittal2013}, we prefer to transform the problem into a submodular maximization one, where we can use a greedy algorithm to produce a solution with some optimality guarantee.
	
%	Since all the requests are well-routed, in particular, there is always a source node at the end of each path which has stored the content object indefinitely, we can assume that there exists an initial feasible content placement with associated cost $C_0:=C(X_0) <\infty$. We will talk about this initial content placement later. Since we will only look at greedy schemes, and $C(X)$ is non-increasing, then, $C_0$ is an upper-bound on the aggregate cost, $C(X)$. Following \cite{sigmetrics}, we can find an allocation which maximizes the caching gain defined by
%	\begin{equation}
%	F(X)= C_0 - C(X), \label{eq:F_X}
%	\end{equation}
%	which is the expected cost reduction obtained by caching at intermediate nodes along the paths. Then we can formulate our optimization problem as
%	

\section{Continuous-Greedy Algorithm}\label{sec:contgreed}
The \emph{continuous-greedy} algorithm by  Calinescu et al.~\cite{calinescu2011} attains a tighter guarantee than the greedy algorithm, raising the approximation ratio from $0.5$ to $1-1/e\approx 0.63$. The algorithm maximizes the so-called  \emph{multilinear extension} of objective $F$, thereby obtaining a fractional solution $Y$ in the convex hull of the constraint space. The resulting solution is then rounded to produce an integral solution.


	
	\begin{algorithm}[!t]
		\caption{Continuous-Greedy}\label{alg:cg}
\begin{scriptsize}
		\begin{algorithmic}[1]
			\REQUIRE $G:\tilde{\domain}\to\reals_+$, $\mathbf{x}_0$, stepsize $0<\gamma\leq 1$
			\STATE  $t \leftarrow 0, k\leftarrow 0\; \mathbf{y}_0\leftarrow \mathbf{x}_0$
			\WHILE{$t <1$}
			\STATE  $\mathbf{m}_k \leftarrow \mathop{\arg\max}_{\mathbf{m}\in \tilde{\domain}} \langle \mathbf{m},\nabla G(\mathbf{y}_k)\rangle\;$ 
			\STATE $\gamma_k\leftarrow \min\{\gamma,1-t\}\;$
			\STATE $\mathbf{y}_{k+1}\leftarrow \mathbf{y}_k+\gamma_k\mathbf{m}_k, t\leftarrow t+\gamma_k, k\leftarrow k+1\;$
			\ENDWHILE
			\RETURN $\mathbf{y}_k\;$
		\end{algorithmic}
\end{scriptsize}
	\end{algorithm}


\subsection{Algorithm Overview} Formally, the multilinear extension of the caching gain $F$  is defined as follows. Define the convex hull of the set defined by the constraints \eqref{eq:fcon} in \textsc{MaxCG} as:
 \begin{align}\!\!\!\tilde{\domain} = \conv ( \{\mathbf{x} %\in \{0,1\}^{|V||\catalog|}\!\! 
 : \mathbf{x}\in \domain, \mathbf{x}\geq \mathbf{x}_0  \} )  \subseteq[0,1]^{|V||\mathcal{C}|}\label{eq:hull}\end{align}
 Intuitively, $\mathbf{y}\in \tilde{\domain}$ is a \emph{fractional} vector in $\reals^{|V||\domain|}$ satisfying the capacity constraints, and the bound $\mathbf{y}\geq \mathbf{x}_0$.

%$\mathbf{y}\in \tilde{\domain}$ is a fractional vector in $\reals^{|V||\domain|}$  satisfying the following set of constraints:
%	\begin{subequations}\label{eq:D}
%		\begin{align}
%		&\textstyle \sum_{i\in\catalog} y_{vi} \leq c_v, \qquad \text{for all } v\in V,\\
%		&y_{vi}\in [0,1], \qquad\text{for all } v\in V, i\in \mathcal{C}, \text{ and}\\
 %               &\mathbf{y} \geq \mathbf{x}_0.
%		\end{align}
%	\end{subequations}
 % both the capacity constraints as well as the bound $\mathbf{y}\geq \mathbf{x}_0.$, with the integrality constraints relaxed.
 Given a $\mathbf{y}\in \tilde{\domain}$, consider a random vector $\mathbf{x}$ in $\{0,1\}^{|V||\mathcal{C}|}$ generated as follows: for all $v\in V$ and $i \in \catalog$, the coordinates $x_{vi}\in\{0,1\}$  are independent Bernoulli  variables such that  $\prob(x_{vi}=1)=y_{vi}$. The multilinear extension $G:\tilde{\domain}\to \reals_+$ of $F:\domain_{\bm{\lambda}}\to\reals_+$ is defined via  following expectation $G(\mathbf{y}) = \mathbb{E}_{\mathbf{y}}[F(\mathbf{x})]$, parameterized by $\mathbf{y}\in\tilde{\domain}$, i.e.,
	\begin{equation}
	\label{eq:multilinearEx}
	G(\mathbf{y})  = \!\!\!\! \sum\limits_{\mathbf{x}\in \{0,1\}^{|V||\mathcal{C}|}}\!\!\!\!\!\!F(\mathbf{x}) \times\!\!\!\! \prod_{(v,i)\in V\times \catalog}\!\!\!\!\!y_{vi}^{x_{vi}}(1-y_{vi})^{1-x_{vi}},\!\!
	\end{equation}


The continuous-greedy algorithm, summarized in Alg.~\ref{alg:cg}, proceeds by first producing a fractional vector $\mathbf{y}\in \tilde{\domain}$. Starting from $\mathbf{y}_0=\mathbf{x}_0$, the algorithm iterates over: %\footnote{The iteratative steps \eqref{eq:its} are related to the so-called conditional gradient/Frank-Wolfe algorithm \cite{Bian-CSM,frank-wolfe} in constrained optimization.}:
\begin{subequations}\label{eq:its}
\begin{align}
	\mathbf{m}_k &\in \textstyle\mathop{\arg\max}_{\mathbf{m}\in\tilde{\domain}} \langle \mathbf{m}, \nabla G(\mathbf{y}_k)\rangle, \label{eq:maxlin}\\
        \mathbf{y}_{k+1} &= \mathbf{y}_k + \gamma_k \mathbf{m}_k,
\end{align} 
\end{subequations}
for an appropriately selected step size $\gamma_k\in [0,1]$. Intuitively, this yields an approximate solution to the non-convex problem:
\begin{subequations}\label{eq:nonconv}
\vspace*{-5mm}
 \begin{align}
\text{Maximize:} &\quad G(\mathbf{y})\\
\text{subj.~to:} & \quad \mathbf{y}\in\tilde{\domain}.
\end{align}
\end{subequations}
%\si{Are we still talking about Frank-Wolfe?}
 %In particular, step~\eqref{eq:maxlin} is essentially the conditional gradient--a.k.a.~Frank-Wolfe~\cite{Bian-CSM,nlp}--method. 
Even though \eqref{eq:nonconv} is not  convex, the output of Alg.~\ref{alg:cg} is  within a $1-1/e$ factor from the optimal solution $\mathbf{y}^*\in \tilde{\domain}$ of \eqref{eq:nonconv}. This fractional solution can  be rounded  to produce a solution to \textsc{MaxCG} with the same approximation guarantee using  either the pipage rounding \cite{ageev2004pipage} or the swap rounding \cite{calinescu2011,chekuri2010dependent} schemes: \techrep{we review both  in Appendix~\ref{sec:rounding}.}{ we refer the reader to  \cite{techrep} for details.}

\begin{comment}
Note that the maximization in \eqref{eq:maxlin} is a Linear Program (LP): it involves maximizing a linear objective subject to a set of linear constraints, and can thus be computed in polynomial time. However, this presumes access to the gradient $\nabla G$.   On the other hand, the expectation $G(\mathbf{y})=\expect_\mathbf{y}[F(\mathbf{x})]$ alone, given by \eqref{eq:multilinearEx}, involves a summation over $2^{|V||\catalog|}$ terms, and it may not be easily computed in polynomial time. To address this, the customary approach is to produce random samples  $\mathbf{x}$ and use these to produce an unbiased estimate of the gradient; this estimate can be used in Alg.~\ref{alg:cg} instead of the gradient. As we discuss below, Alg.~\ref{alg:cg}  still produces a solution that is within $1-1/e$ from the optimal, with high probability (c.f.~Section~\ref{sec:sample}). Nevertheless, we show below that \textsc{MaxCG} exhibits additional structure, which can be used to construct a polynomial-time estimator of the gradient $\nabla G(\mathbf{y})$ that  \emph{eschews sampling altogether}, by using the Taylor expansion of $G$.

Before presenting our estimator tailored to \textsc{MaxGC}, we first describe the sampling-based estimator used in the existing literature for the (general-purpose)  continuous-greedy algorithm.
\end{comment}
%\subsection{Sampling-Based Estimator}\label{sec:sample}
\noindent\textbf{A Sampling-Based Estimator.}\label{sec:sample}
Function $G$, given by \eqref{eq:multilinearEx}, involves a summation over $2^{|V||\catalog|}$ terms, and cannot be easily computed in polynomial time. 
Typically, a sampling-based estimator (see, e.g., \cite{calinescu2011})  is used instead.  Function $G$ is linear when restricted to each coordinate $y_{vi}$, for some $v\in V$, $i\in \catalog$ (i.e., when all  inputs except $y_{vi}$ are fixed). As a result, the partial derivative of $G$ w.r.t. $y_{vi}$ can be written as:
	\begin{align}\label{eq:deriv_G}
%	\begin{split}
\textstyle	\frac{\partial G(\mathbf{y})}{\partial y_{vi}}& = \mathbb{E}_{\mathbf{y}}[F(\mathbf{x})|x_{vi}=1]- \mathbb{E}_{\mathbf{y}}[F(\mathbf{x})|x_{vi}=0]\geq 0,%\\&= \mathbb{E}[C(\mathbf{x})|x_{vi}=0] - \mathbb{E}[C(\mathbf{x})|x_{vi}=1]\geq 0,
%	\end{split}
	\end{align} 
	where the last inequality is due to monotonicity of $F$. One can thus estimate the gradient by %by computing the expectation of $F(\mathbf{x})$ when all other Bernoulli coordinates are sampled independently with probabilities determined by $\mathbf{y}$, and $x_{vi}$ is set to 1 and 0, respectively; the difference of the two expectations yields an unbiased estimator of $\frac{\partial G(\mathbf{y})}{\partial y_{vi}}$.
%In turn, this suggests the following sampling-based estimator for the gradient $\nabla G(\mathbf{y})$: First,
(a) producing $T$ random samples $\mathbf{x}^{(\ell)}$, $\ell=1,\ldots,T$ of the random vector $\mathbf{x}$, consisting of independent Bernoulli coordinates,  and (b) computing, for each pair $(v,i)\in V\times \catalog$, the average
\begin{align}\textstyle
\widehat{\frac{\partial G(\mathbf{y})}{\partial y_{vi}}} = 
\frac{1}{T} \sum_{\ell=1}^T \left( F([\mathbf{x}^{\ell}]_{+(v,i)} )-F([\mathbf{x}^{\ell}]_{-(v,i)})\right),\label{eq:samplestimator}
\end{align}
where $[\mathbf{x}]_{+(v,i)}$,$[\mathbf{x}]_{-(v,i)}$ are equal to vector $\mathbf{x}$ with the $(v,i)$-th coordinate set to 1 and 0, respectively. Using this estimate, Alg.~\ref{alg:cg} \techrep{}{is poly-time and}
 attains an approximation ratio arbitrarily close to $1-1/e$ for appropriately chosen $T$\techrep{.}{ (see \cite{techrep} for a formal guarantee and characterization of Alg.~\ref{alg:cg}'s complexity).}
\techrep{
In particular, the following theorem holds:
\begin{theorem}\label{thrm:sampling}[Calinescu et al.~\cite{calinescu2011}] Consider Alg.~\ref{alg:cg}, with $\nabla G(\mathbf{y}_k)$ replaced by the sampling-based estimate $\widehat{\nabla G(\mathbf{y}^k)}$, given by \eqref{eq:samplestimator}. Set $T = \frac{10}{\delta^2}(1+\ln (|\catalog||{V}|))$, and $\gamma=\delta$, where $\delta = \frac{1}{40|\catalog||{V}|\cdot(\sum_{v\in{V}}c_v)^2}.$ Then, the algorithm terminates after $K=1/\gamma=1/\delta$ steps and, with high probability, 
$$G(\mathbf{y}^K) \geq (1-(1-\delta)^{1/\delta}) G(\mathbf{y}^*) \geq (1-1/e)G(\mathbf{y}^*),$$
where $\mathbf{y}^*$ is an optimal solution to \eqref{eq:nonconv}.
\end{theorem}
The proof of the theorem can be found  in Appendix A of Calinescu et al.~\cite{calinescu2011} for general submodular functions over arbitrary matroid constraints; we state Thm.~\ref{thrm:sampling} here with constants $T$ and $\gamma$ set specifically for our objective $G$ and our set of constraints $\tilde{D}$.}{}

\techrep{Under this parametrization of $T$ and $\gamma$, Alg.~\ref{alg:cg} runs in polynomial time.  More specifically, note that $1/\delta=  O(|\catalog||{V}|\cdot(\sum_{v\in{V}}c_v)^2)$ is polynomial in the input size. Moreover, the algorithm runs for $K =1/\delta$ iterations in total. Each iteration requires $T = O(\frac{1}{\delta^2}(1+\ln (|\catalog||V|)$ samples, each involving a polynomial computation (as $F$ can be evaluated in polynomial time). Finally, LP \eqref{eq:maxlin} can be solved in polynomial time in the number of constraints and variables, which are $O(|V||\catalog|)$.}{}
 


%Then, the following theorem holds:
%\begin{theorem}\label{thrm:sampling}[Calinescu et al.~\cite{calinescu2011}] Consider Alg.~\ref{alg:cg}, with $\nabla G(\mathbf{y}_k)$ replaced by the sampling-based estimate $\widehat{\nabla G(\mathbf{y}^k)}$, given by \eqref{eq:samplestimator}. Set $T = \frac{10}{\delta^2}(1+\ln (|\catalog||{V}|))$, and $\gamma=\delta$, where $\delta = \frac{1}{40|\catalog||{V}|\cdot(\sum_{v\in{V}}c_v)^2}.$ Then, the algorithm terminates after $K=1/\gamma=1/\delta$ steps and, with high probability, 
%$$G(\mathbf{y}^K) \geq (1-(1-\delta)^{1/\delta}) G(\mathbf{y}^*) \geq (1-1/e)G(\mathbf{y}^*),$$
%where $\mathbf{y}^*$ is an optimal solution to \eqref{eq:nonconv}.
%\end{theorem}
%The proof of the theorem can be found  in Appendix A of Calinescu et al.~\cite{calinescu2011} for general submodular functions over arbitrary matroid constraints; we state it here with constants $T$ and $\gamma$ set specifically for our objective $G$ and our set of constraints $\tilde{D}$. 
%
%Under this parametrization of $T$ and $\gamma$, Alg.~\ref{alg:cg} runs in polynomial time.  More specifically, note that $1/\delta=  O(|\catalog||{V}|\cdot(\sum_{v\in{V}}c_v)^2)$ is polynomial in the input size. Moreover, the algorithm runs for $K =1/\delta$ iterations in total. Each iteration requires $T = O(\frac{1}{\delta^2}(1+\ln (|\catalog||V|)$ samples, each involving a polynomial computation (as $F$ can be evaluated in polynomial time). Finally, LP \eqref{eq:maxlin} can be solved in polynomial time in the number of constraints and variables, which are $O(|V||\catalog|)$.
 
\subsection{A Novel Estimator via Taylor Expansion}\label{sec:taylor}

The classic approach to estimate the gradient via sampling has certain drawbacks.  The number of samples $T$ required to attain the $1-1/e$ ratio is quadratic in $|V||\catalog|$. In practice, even for networks and catalogs of moderate size (say, $|V|=|\catalog|=100$), the number of samples becomes prohibitive (of the order of $10^8$). Producing an estimate for $\nabla G$ via a closed form computation that eschews sampling thus has significant computational advantages. In this section, we show that the multilinear relaxation of the caching gain $F$ admits  such a closed-form characterization.

  We say that a polynomial $f:\reals^d\to\reals$ is in  \emph{Weighted Disjunctive Normal Form} (\emph{W-DNF}) if it can be written as
\begin{align}
	f(\mathbf{x}) = \textstyle\sum_{s\in \mathcal{S}}\beta_s \cdot \prod_{j\in \mathcal{I}(s)}(1-x_j),\label{wdnf}
\end{align}
for some index set $\mathcal{S}$, positive coefficients $\beta_s>0$, and index sets $I(s)\subseteq \{1,\ldots, d\}$. Intuitively,  treating binary variables $x_j\in \{0,1\}$ as boolean values,  each W-DNF polynomial can be seen as a weighted  sum (disjunction) among products (conjunctions) of negative literals.  
These polynomials  arise naturally in the context of our problem; in particular:
\begin{lemma}\label{wdnfmoments}
For all $k\geq 1$, $\mathbf{x}\in \mathcal{D}$, and $e\in E$,  $\rho^k_e(\mathbf{x},\bm{\lambda})$ is a W-DNF polynomial whose coefficients depend on $\bm{\lambda}$.
\end{lemma}
\begin{proof}[Proof (Sketch)]
The lemma holds for $k=1$ by \eqref{lamr} and \eqref{eq:rho_X}. The lemma follows by induction, as W-DNF polynomials over binary  $\mathbf{x}\in \mathcal{D}$ are closed under multiplication; this is because $(1-x)^\ell=(1-x)$ for all $\ell\geq 1$ when $x\in\{0,1\}$.
\end{proof}
  Hence, \emph{all load powers are W-DNF polynomials}\techrep{; a detailed proof be found in Appendix~\ref{app:wdnfmomentslemma}}{}.
Expectations of  W-DNF polynomials have a remarkable property:
\begin{lemma}\label{lemma:compute} Let  $f:\domain_{\bm{\lambda}}\to\reals$ be a W-DNF polynomial, and let $\mathbf{x}\in \domain$ be a random vector of independent Bernoulli coordinates parameterized by $\mathbf{y}\in \tilde{\domain}$. Then $\expect_{\mathbf{y}}[f(\mathbf{x})]=f(\mathbf{y})$, where $f(\mathbf{y})$ is the evaluation of the W-DNF polynomial representing $f$ over the real vector $\mathbf{y}$.  
\end{lemma} 
\techrep{
\begin{proof}
As $f$ is W-DNF, it can be written as 
\begin{align*}f(\mathbf{x})=\sum_{s\in \mathcal{S}}\beta_s \prod_{t\in \mathcal{I}(s)}(1-x_t)
\end{align*}
for appropriate $\mathcal{S}$, and appropriate $\beta_s,\mathcal{I}(s)$, where $s\in\mathcal{S}$. Hence,
\begin{align*}\expect_{\mathbf{y}}[f(\mathbf{x})]&=\sum_{s\in \mathcal{S}}\beta_s \expect_{\mathbf{y}}\left[\prod_{t\in \mathcal{I}(s)}(1-x_t)\right]\\
& = \sum_{s\in \mathcal{S}}\beta_s \prod_{t\in \mathcal{I}(s)}(1-\expect_{\mathbf{y}}[x_t]), \text{ by independence}\\
& = \sum_{s\in \mathcal{S}}\beta_s \prod_{t\in \mathcal{I}(s)}(1-y_t).\qedhere
\end{align*}
\end{proof}
}{
\begin{proof}
%As $f$ is W-DNF, it can be written as 
%\begin{align*}f(\mathbf{x})=\sum_{r\in \mathcal{S}}\beta_r \prod_{t\in \mathcal{I}(r)}(1-x_t)
%\end{align*}
%for appropriate $\mathcal{S}$, and appropriate $\beta_r,\mathcal{I}(r)$, for $r\in\mathcal{S}$. Hence,
By \eqref{wdnf} and independence, we have
%\begin{align*}
$\expect_{\mathbf{y}}[f(\mathbf{x})]=\sum_{s\in \mathcal{S}}\beta_s \expect_{\mathbf{y}}\left[\prod_{t\in \mathcal{I}(s)}(1-x_t)\right] %\\
 = \sum_{s\in \mathcal{S}}\beta_s \prod_{t\in \mathcal{I}(s)}(1-\expect_{\mathbf{y}}[x_t]) %, \text{ by independence}\\
 = \sum_{s\in \mathcal{S}}\beta_s \prod_{t\in \mathcal{I}(s)}(1-y_t).$%\qedhere
%\end{align*}
\end{proof}}

Lemma~\ref{lemma:compute} states that, to compute the expectation of a W-DNF polynomial $f$ over i.i.d.~Bernoulli variables with expectations $\mathbf{y}$, it suffices to \emph{evaluate $f$ over input $\mathbf{y}$}. Expectations computed this way therefore do not require sampling. %\techrep{The proof can be found in Appendix~\ref{proofoflemma:compute}.}{} 



We  leverage this property to approximate $\nabla G(\bm{y})$ by taking the Taylor expansion of the cost functions $C_e$ at each edge $e\in E$. This allows us to write $C_e$ as a power series w.r.t.~$\rho_e^k$, $k\geq 1$; from Lemmas~\ref{wdnfmoments} and~\ref{lemma:compute}, we can compute the expectation of this series in a closed form. In particular, by expanding the series and rearranging terms it is easy to show the following\techrep{ lemma, which is proved in Appendix~\ref{proofoftaylorlemma}}{}:
\begin{lemma}\label{taylorlemma}
 Consider a cost function $C_e:[0,1)\to\reals_+$ which satisfies Assumption~\ref{as:conv} and for which the Taylor expansion exists at some $\rho^*\in[0,1)$. Then, for  $\mathbf{x} \in \domain$ a random Bernoulli vector parameterized by $\mathbf{y}\in \tilde{\domain}$,
\begin{align}
\!\!\!\frac{\partial G(\mathbf{y})}{\partial y_{vi}} \!\!\approx\!\!
\sum_{e\in E}\! \sum_{k=1}^{L}\!\alpha^{(k)}_e \!\!\left[\rho^k_e\left([\mathbf{y}]_{-(v,i)},\!\bm{\lambda}\right) \!-\!\rho^k_e\left([\mathbf{y}]_{+(v,i)},\!\bm{\lambda}\right)\right]\!\!\!%\nonumber\\
%&\quad+ o((\rho-\rho^*)^L)
\label{eq:taylorapprox2}
\end{align}
where, 	$\textstyle\alpha^{(k)}_e  = \sum_{i=k}^{L} \frac{(-1)^{i-k}\binom{i}{k}}{i!}C^{(i)}_{e}(\rho^*)(\rho^*)^{i-k}$  for $k=0,1,\cdots,L,$ and the error of the approximation is:
%\begin{align*}
$\textstyle\frac{1}{(L+1)!}\sum_{e\in E}C^{(L+1)}_{e}(\rho') \Big[ \expect_{[\mathbf{y}]_{-{v,i}}}[(\rho_e(\mathbf{x},\bm{\lambda})-\rho^*)^{L+1}] %\\
\textstyle-  \expect_{[\mathbf{y}]_{+{v,i}}}[(\rho_e(\mathbf{x},\bm{\lambda})-\rho^*)^{L+1}]\Big]. $%\end{split}\end{align*}


%and  $\rho^k_e$ corresponds to the W-DNF polynomial representing the $k$-th power of $\rho_e$, evaluated over the fractional variables $\mathbf{y}$, with $y_{vi}$ set to 0 and 1 for each of the two terms in \eqref{eq:taylorapprox2}. 
\end{lemma}
 Estimator \eqref{eq:taylorapprox2} is \emph{deterministic}: no random sampling is required. Moreover, Taylor's theorem allows us to characterize the error  (i.e., the \emph{bias}) of this estimate. We use this to characterize the final fractional solution $\mathbf{y}$ produced by Alg.~\ref{alg:cg}:
  	\begin{theorem}\label{theorem:converge}
	     Assume that all $C_e$, $e\in E$, satisfy Assumption~\ref{as:conv}, are $L+1$-differentiable, and that all their $L+1$ derivatives are bounded by $W\geq 0$. Then, consider Alg.~\ref{alg:cg}, in which $\nabla G(\mathbf{y}_k)$ is estimated via the Taylor estimator \eqref{eq:taylorapprox2}, where each edge cost function is approximated at $\rho_e^* = \expect_{\mathbf{y}_k}[\rho_e(\mathbf{x},\bm{\lambda})]=\rho_e(\mathbf{y}_k,\bm{\lambda}).$
Then,  % of the algorithm, 
%		For a continuous submodular objective function $G$ with $L$-Lipschitz continuous gradient, we are given an estimator $z=[z_{vi}]_{v\in V,i\in \mathcal{C}}\in \mathbb{R}^{|V||\mathcal{C}|}$, where  $|\mathbb{E}\left[z|\mathbf{y}\right] -\triangledown G(\mathbf{y})|\leq B$, and, $\mathbb{E}\left[||z||_2^2|\mathbf{y}\right]\leq \sigma^2$.
%		For a given number of iterations $K$, or alternatively, for a given constant stepsize $\gamma= K^{-1}$, Algorithm \ref{alg:caching} produces the following optimality guarantee:	
		\begin{equation}\label{eq:optimal}
		\textstyle G(\mathbf{y}_{K}) \geq (1-\frac{1}{e})G(\mathbf{y}^*) - 2D B- \frac{P}{2K},
		\end{equation}
		where  $K=\frac{1}{\gamma}$ is the number of iterations, $\mathbf{y}^*$ is an optimal solution to \eqref{eq:nonconv},  
$D = \max_{\mathbf{y}\in \tilde{\domain}} \|\mathbf{y}\|_2\leq |V|\cdot\max\limits_{v\in{V}}c_v,$ is the diameter of  $\tilde{\domain}$, $B\leq \frac{W|E|}{(L+1)!}$ is the bias of estimator \eqref{eq:taylorapprox2}, and $P=2C(\mathbf{x}_0),$ is a Lipschitz constant of $\nabla G$.
	\end{theorem}
	\techrep{The proof can be found in Appendix~\ref{app:3}.}{} The theorem immediately implies that we can replace \eqref{eq:taylorapprox2} as an estimator in Alg.~\ref{alg:cg}, and attain an approximation arbitrarily close to $1-1/e$. 


	\noindent\textbf{Estimation via Power Series.} For arbitrary $L+1$-differentiable cost functions $C_e$, the estimator \eqref{eq:taylorapprox2} can be leveraged by replacing $C_e$ with its Taylor expansion. In the case of queue-dependent cost functions, as described in Example 4 of Section~\ref{sec:mincost}, the power-series \eqref{eq:power} can be used instead. For example, the expected queue size (Example 1, Sec.~\ref{sec:mincost}), is given by $C_e(\rho_e) = \frac{\rho_e}{1-\rho_e} =\sum_{k=1}^\infty \rho_e^k.$
In contrast to the Taylor expansion, this power series does not depend on a point $\rho^*_e$ around which the function $C_e$ is approximated.

\begin{comment}
	\begin{equation}
		(f_1 * f_2)(\mathbf{x}) = \sum_{j\in \mathcal{J},j'\in \mathcal{J}'}\alpha_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cup \mathcal{I}'(j')}(1-x_t).
	\end{equation}



	To obtain a tighter optimality gap for the submodular maximization problem that the one attained the greedy algorithm, Calinescu et al. \cite{calinescu2011} propose to relax the objective set function $F(\mathbf{x})$  via its \emph{multilinear extension} which transforms it into a continuous-submodular objective function $G(\mathbf{y})$. By optimizing for $G(\mathbf{y})$ subject to the relaxed feasibility region, using continuous greedy algorithm \cite{calinescu2011}, %or more recently proposed Frank-Wolfe algorithm \cite{Bian-CSM},
 it can be shown that each of these algorithms can reach a tighter approximation than the greedy algorithm. More specifically, each algorithm obtains an approximate solution within $1-1/e \simeq 63\%$ from the optimal solution. 
%	\subsection{Multilinear Extension}

	We can obtain the multilinear extension for a monotone submodular function $F: 2^{|V||\mathcal{C}|}\rightarrow \mathbb{R}_+$ as follows:

	We denote by $F_{\mathbf{x}}(v,i)$ to be the caching gain induced by adding object $i$ at node $v$. Hence,  
	\begin{eqnarray*}\label{eq:F_deriv}
		\mathbb{E}[F_{\mathbf{x}}(v,i)] &=& \mathbb{E}[F(\mathbf{x})|x_{vi}=1]- \mathbb{E}[F(\mathbf{x})|x_{vi}=0]\\&=& \frac{\partial G}{\partial y_{vi}}.
	\end{eqnarray*}


	Similarly, $\frac{\partial^2 G}{\partial y_{vi}^2} = 0$. For $(v_1,i_1)\neq(v_2,i_2)$,  we can compute the second derivative of $G$ \cite{calinescu2011} as given by
	\begin{IEEEeqnarray*}{+rCl+x*}
		\frac{\partial^2 G}{\partial y_{v_1i_1}\partial y_{v_2i_2}} &=& \mathbb{E}[C(\mathbf{x})|x_{v_1i_1}=1,x_{v_2i_2}=0]\\ &+&\mathbb{E}[C(\mathbf{x})|x_{v_1i_1}=0,x_{v_2i_2}=1] \\&-&\mathbb{E}[C(\mathbf{x})|x_{v_1i_1}=1,x_{v_2i_2}=1]\\ &-& \mathbb{E}[C(\mathbf{x})|x_{v_1i_1}=0,x_{v_2i_2}=0] \leq 0,
	\end{IEEEeqnarray*}
	which is $\leq 0$ due to the supermodularity of $C(\mathbf{x})$. Hence, $G(\mathbf{y})$ is continuous submodular.
	



	In additions, it is easy to see that for the stable network operating regime, $||G||$, $||\triangledown G||$, and $||\triangledown^2 G||$ are bounded by $C_0$, $C_0$ and $2C_0$, respectively. Consequently, $G$ and $\triangledown G$ are $L$-Lipschitz continuous, with $L =2C_0$. 
	
	%	\subsection{Network Initialization}
	%	Using the multilinear extension technique, the domain of the problem is transfered from $X \in \{0,1\}^{|V|\times|\mathcal{C}|}$ to $Y \in [0,1]^{|V|\times|\mathcal{C}|}$. Furthermore, $G(Y) = C_0 - \mathbb{E}[C(X)]$. Suppose we are given an initial content marginal probability matrix $Y_0$ with property $\mathbb{E}[\rho_{u,v}(X)] = \rho_{u,v}(Y)<1$, for all $(u,v)\in E$. Then, we are assured that there exists a content placement matrix $X_0$ which can be obtained by rounding 
	\subsection{Offline Algorithm}
	Consider now the problem 
	\begin{subequations}\label{eq:opt_Y}
		\begin{equation}
		\max G(\mathbf{y})
		\end{equation}
		\begin{equation}
		\text{subject to: } \mathbf{y}\in \mathcal{D},
		\end{equation}
	\end{subequations}
	where $\mathcal{D}$ is the set of vectors $\mathbf{y}=[y_{vi}]_{v\in V, i\in \mathcal{C}}$ satisfying
	\begin{subequations}\label{eq:D}
		\begin{equation}
		\sum_{i\in\mathcal{C}} y_{vi} \leq c_v, \qquad v\in V,
		\end{equation}
		\begin{equation}
		y_{vi}\in [0,1], \qquad\forall v\in V, i\in \mathcal{C},
		\end{equation}
	\end{subequations}
	The offline algorithm, described in Algorithm \ref{alg:caching} \cite{Bian-CSM}, assumes that there is a Central Logic Unit (CLU) in the network with global view of the request arrival vector $\mathcal{R}$, the network topology, the content marginal probability vector $\mathbf{y}$,  and its corresponding content placement vector $\mathbf{x}$ at each step. 
	
	In the initial phase of Algorithm 
	We note that given $\mathcal{R}$, and $\mathbf{x}$, one can compute $F(\mathbf{x})$ with run time $O(|E||\mathcal{R}|)$. However, we need an exponential number of evaluations of $F(\mathbf{x})$ to compute $G(\mathbf{y})$ (or its gradient) deterministically. Alternatively, since $\mathbf{x}$ is a random content placement vector where each element $x_{vi}$ is independently rounded to 1 with probability $y_{vi}$ or 0 otherwise, the CLU can estimate $\frac{\partial G}{\partial y_{vi}}$ for each $(v,i), v\in V, i\in \mathcal{C}$, by computing $F_{\mathbf{x}}(v,i)$ with independent samples of $\mathbf{x}$. In particular, let $Z =[z_{vi}] \in \mathbb{R}^{|V||\mathcal{C}|}$ be an estimate of $\triangledown G(\mathbf{y})$, where $z_{vi}$ is an estimate of $\mathbb{E}[F_{\mathbf{x}}(v,i)]$, obtained by averaging over $T$ evaluations $F_{\mathbf{x}}(v,i)$ with independent samples of $\mathbf{x}$. 
	
	
	%	We prove the optimality guarantee of Algorithm \ref{alg:caching}, in Section \ref{sec:converge}, Theorem \ref{theorem:converge}, for the online case where there are some restrictions involved. The result of Theorem \ref{theorem:converge} is directly applicable to the offline case by setting $\epsilon = 0$ in \eqref{eq:optimality}. In particular, we have the following corollary.
	\subsection{Convergence Analysis}
	\label{sec:converge}
	In this section, we describe the convergence of Algorithm \ref{alg:caching}. It is worth noting that our analysis extends the results in \cite{Bian-CSM} for stochastic problems. To study the stochasticity of the problem, we use the model introduced by Nemirovski \cite{nemirovski-efficient}. In particular, note that the search trajectory of the proposed algorithm at $k$th iteration is governed by random vector $\mathbf{x}_k$, and hence, it is random as well. That is,
	\begin{equation}\label{eq:Y_X}
	\mathbf{y}_k=\mathbf{y}_k(\mathbf{x}^{k-1}),\qquad \mathbf{x}^k:=(\mathbf{x}_1,\cdots,\mathbf{x}_k).
	\end{equation}
	
	Following the argument in \cite{Bian-CSM}, we introduce univariate auxiliary function $g_{\mathbf{y},\mathbf{m}}(\xi):=G(\mathbf{y}+ \xi \mathbf{m}),\xi \in [0,1], \mathbf{m}\in[0,1]^{|V||\mathcal{C}|}$. Since $G(\mathbf{y})$ is component-wise concave, then, $g_{\mathbf{y},\mathbf{m}}(\xi)$ is concave in $[0,1]$. It is easy to see that for a stable initial network operating regime, $\frac{d g_{\mathbf{y},\mathbf{m}}(\xi)}{d \xi}$ is $L$-Lipschitz continuous in $[0,1]$. In particular, since $\forall \mathbf{m}\in[0,1]^{|V||\mathcal{C}|}$
	\begin{IEEEeqnarray}{+rCl+x*}
		&\mathbf{m}'\triangledown^2 G(\mathbf{y})\mathbf{m}& =\sum\limits_{(v,i) } \mathbf{m}_{(v,i)}^2\frac{\partial^2 G}{\partial y_{vi}^2} \nonumber\\+&\sum_{(v_1,i_1)\neq (v_2,i_2)}& \mathbf{m}_{(v_1,i_1)}\mathbf{m}_{(v_2,i_2)}\frac{\partial^2 G}{\partial y_{v_1i_1}\partial y_{v_2i_2}} \nonumber \\
		& & \geq  -2C_0.
	\end{IEEEeqnarray}
	we can set $L=2C_0$.
	
	Now we can formulate the proof of the convergence of Algorithm \ref{alg:caching} in the following theorem.
	\begin{theorem}\label{theorem:converge}
		For a continuous submodular objective function $G$ with $L$-Lipschitz continuous gradient, we are given an estimator $z=[z_{vi}]_{v\in V,i\in \mathcal{C}}\in \mathbb{R}^{|V||\mathcal{C}|}$, where  $|\mathbb{E}\left[z|\mathbf{y}\right] -\triangledown G(\mathbf{y})|\leq B$, and, $\mathbb{E}\left[||z||_2^2|\mathbf{y}\right]\leq \sigma^2$.
		For a given number of iterations $K$, or alternatively, for a given constant stepsize $\gamma= K^{-1}$, Algorithm \ref{alg:caching} produces the following optimality guarantee:	
		\begin{equation}\label{eq:optimal}
		\mathbb{E}[G(\mathbf{y}_{K})] \geq (1-\frac{1}{e})G(\mathbf{y}^*) - D (\sigma+B)- \frac{L}{2K},
		\end{equation}
		where $\mathbf{y}^*$ is an optimal solution to \eqref{eq:opt_Y}, and $D$ is the diameter of the feasible region.
	\end{theorem}


	\begin{proof}
		See Appendix \ref{app:3}
	\end{proof}
	\subsection{Unbiased Estimator}
	Suppose we have a random unbiased estimator, i.e., $B = 0$. As shown in \eqref{eq:optimal},  the optimality gap can be improved by increasing $K$ and decreasing $\sigma$. To decrease the estimator variance $\sigma$, the CLU can increase the number of independent evaluations of $F_{\mathbf{x}}(v,i)$, denoted by $T$. It can be easily verified that $\sigma \propto 1/\sqrt{T}$, hence, we can tune the number of evaluations to control the error on the optimality gap.
	\begin{cor}
		Suppose we have a continuous submodular objective function $G$ with Lipschitz continuous gradient, and an unbiased estimator, where we take the average of $T$ samples of gradient at each iteration. After $K$ iterations, Algorithm \ref{alg:caching} produces the following asymptotic optimality guarantee, when $T\rightarrow \infty$, $K\rightarrow \infty$. 
		\begin{equation}\label{eq:optimal2}
		\mathbb{E}[G(\mathbf{y}_{K})] \geq (1-\frac{1}{e})G(\mathbf{y}^*).
		\end{equation}
	\end{cor}
	In particular, it has been shown in Appendix A of \cite{calinescu2011}, that by allowing $T = \frac{10}{\delta^2}(1+\ln (|\catalog||{V}|))$, and $K = 1/\delta$, where $$\delta = \frac{1}{40|\catalog||{V}|\cdot(\sum_{v\in{V}}c_v)^2},$$
	we can have the clean optimality bound given in \eqref{eq:optimal2}.
	%	With this idea in mind, the continuous greedy algorithm works as follows \cite{calinescu2011}: 
	%	\begin{enumerate}
	%		\item   Let $\sigma = \frac{1}{40|V||\mathcal{C}|d^2}$, where $d = \sum\limits_{v in V} c_v$ is the rank of the partition matroid. Start with $t = 0$ and $y(0) = \mathbf{0}$.
	%		\item Let $X(t)$ be the random content placement matrix where each element $x_{vi}(t)$ is independently rounded to 1 with probability $y_{vi}(t)$ or 0 otherwise. For each $(v,i), v\in V, i\in \mathcal{C}$, let $Z(t) =[z_{vi}] \in \mathbb{R}^{|V|\times|\mathcal{C}|}$ be an estimate of $\triangledown G(Y(t))$, where $z_{vi}(t)$ is an estimate of $\mathbb{E}[F_{X}(v,i)]$, obtained by averaging over $\frac{10}{d^2}(1+\ln (|V||\mathcal{C}|)$ independent samples of $X(t)$. 
	%		\item Let $I(t) = [I_{vi}(t)]\in \{0,1\}^{|V|\times|\mathcal{C}|}$ be a maximum weight feasible set, according to weights $Z(t)$. That is, for each node $v$, sort $Z_{vi}(t)$'s in a descending order. Set $I_{vi}(t) = 1$ for the first $c_v$ content objects $i\in \mathcal{C}$, and set $I_{vi}(t) = 0$ for the rest of $i$'s.
	%		\item Let
	%		\begin{equation}
	%		Y(t+\delta) = Y(t) + \delta \cdot\mathbf{1}_{I(t)}.
	%		\end{equation}
	%		\item $t \leftarrow t+1$; if $t<1$ return to step 2. Otherwise, return $Y(1)$.
	%	\end{enumerate}
	%	
	%	As shown in Appendix A of \cite{calinescu2011}, this algorithm achieves a solution within $1-1/e$ from the optimal value. 
	
	\subsection{Complexity of Algorithm \ref{alg:caching}}
	Algorithm \ref{alg:caching} has a polynomial run-time. More specifically, It takes $O(K)$ iterations for the algorithm to reach $t=1$. At each iteration, it requires $O(T)$ samples of $\mathbb{E}[F_{\mathbf{x}}(v,i)]$'s estimate for each $(v,i)$, each of which has a run-time of $O(|E||\mathcal{R}|)$.	
	\subsection{Pipage Rounding}
	Note that the solution of Frank-Wolfe algorithm, $\mathbf{y}(1)$, is fractional, and hence, it requires a rounding step to produce integer solutions. Pipage Rounding \cite{pipage-Ageev2004} is a simple deterministic rounding procedure of linear relaxations. We informally describe the algorithm, for more rigorous description, see  \cite{pipage-Ageev2004}. At each step of the iteration, Pipage Rounding procedure uses the following property of $G$: given a fractional solution $\mathbf{y}(1) \in \mathcal{D}$, there are at least two fractional variables $y_{vi}$ and $y_{v'i'}$, such that transferring mass from one to the other,$1)$ makes at least one of them 0 or 1, $2)$ the new $\hat{\mathbf{y}}$ remains feasible, and $3)$ $G(\hat{\mathbf{y}}) \geq G(\mathbf{y}(1))$, that is the caching gain at $\hat{\mathbf{y}}$ is at least as good as $\mathbf{y}(1)$. If $\hat{\mathbf{y}}$ does not have any fractional element, it returns $\hat{\mathbf{y}}$.
	
	This procedure has a run-time of $O(|V||\mathcal{C}|)$ \cite{sigmetrics}, and since
	each rounding step can only increase $G$, it follows 
	\begin{equation*}
	\mathbb{E}[G(\hat{\mathbf{y}})]\geq \mathbb{E}[G(\mathbf{y}(1))]  \geq (1-\frac{1}{e})G(\mathbf{y}^*).
	\end{equation*}
\section{Biased Estimator}
In the previous section, we applied the multilinear extension to transform the discrete (set) objective function $F(\mathbf{x})$ to a continuous one, $G(\mathbf{y}) = \mathbb{E}[F(\mathbf{x})]$. We then used an unbiased estimator of $	\frac{\partial G}{\partial y_{vi}}= \mathbb{E}[C(\mathbf{x})|x_{vi}=0] - \mathbb{E}[C(\mathbf{x})|x_{vi}=1]$ to derive the Frank-Wolfe algorithm, given in Algorithm \ref{alg:caching}. 

Due to the complexities of this approach, in this section, we explore an approximation method based on Taylor series of $C_{u,v}(\rho_{u,v})$, for $(u,v) \in E$. As noted before, $C_{u,v}(\rho_{u,v})$ is an strictly increasing and convex cost function of $\rho_{u,v}$. Using Taylor's Theorem and for a $\rho^*_{u,v}\in [0,1)$, we have
\begin{eqnarray*}
	C_{u,v}(\rho_{u,v}) &=& C_{u,v}(\rho^*_{u,v}) + \sum_{k=1}^{L}\frac{1}{k!}C^{(k)}_{u,v}(\rho^*_{u,v})(\rho_{u,v}-\rho^*_{u,v})^k\\& +& 
	\frac{1}{(L+1)!}C^{(L+1)}_{u,v}(\rho'_{u,v})(\rho_{u,v}-\rho^*_{u,v})^{L+1},
\end{eqnarray*}
where $\rho'_{u,v} \in [\rho^*_{u,v},\rho_{u,v}]$. 

By reorganizing the terms, we can have
\begin{equation}
	C_{u,v}(\rho_{u,v}) =  \sum_{k=0}^{L}\alpha^{(k)}_{u,v}\rho_{u,v}^k+ \frac{1}{(L+1)!}C^{(L+1)}_{u,v}(\rho'_{u,v})(\rho_{u,v}-\rho^*_{u,v})^{L+1},
\end{equation}
where 
\begin{equation}
	\alpha^{(k)}_{u,v}  = \sum_{i=k}^{L} \frac{(-1)^{i-k}\binom{i}{k}}{i!}C^{(i)}_{u,v}(\rho^*_{u,v})(\rho^*_{u,v})^{i-k}, k=0,1,\cdots,L.
\end{equation}

Now if we take the expected value of $C_{u,v}(\mathbf{x})$ w.r.t. the marginal probabilities, it follows
\begin{equation}
	\mathbb{E}[C_{u,v}(\mathbf{x})] = \sum_{k=0}^{L}\alpha^{(k)}_{u,v}\mathbb{E}[\rho_{u,v}^k]+ \frac{1}{(L+1)!}C^{(L+1)}_{u,v}(\rho'_{u,v})\mathbb{E}[(\rho_{u,v}-\rho^*_{u,v})^{L+1}].
\end{equation}

It turns out that the $\rho_{u,v}^k(\mathbf{x})$ has a special form. In particular, each $(1-x_{vi})^k = (1-x_{vi})$ for any $k>1, v\in V, i\in \mathcal{C}$. In addition, we can write $\rho_{u,v}^(\mathbf{x})$ as
\begin{equation}
	\rho_{u,v}(\mathbf{x}) = \sum_{j\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j \prod_{t\in \mathcal{I}(j)}(1-x_t),
\end{equation}
for some appropriately chosen $\beta_j$'s. Hence, it be shown that 
\begin{equation}
	\rho_{u,v}^2(\mathbf{x}) = \sum_{j,j'\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cap \mathcal{I}(j')}(1-x_t)^2\prod_{t\in \mathcal{I}(j) \triangle \mathcal{I}(j')}(1-x_t),
\end{equation}
where $\mathcal{I}(j) \triangle \mathcal{I}(j')$ is the symmetric difference of the sets $\mathcal{I}(j) $ and $\mathcal{I}(j')$. Now since $(1-x_t)^2 = (1-x_t)$, it follows
\begin{equation}
	\begin{split}
		\rho_{u,v}^2(\mathbf{x}) = \sum_{j,j'\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cap \mathcal{I}(j')}(1-x_t)\prod_{t\in \mathcal{I}(j) \triangle \mathcal{I}(j')}(1-x_t)\nonumber\\ =\sum_{j,j'\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cup \mathcal{I}(j')}(1-x_t).
	\end{split}
\end{equation}

Since $x_{vi}$'s are independent random variables, the expected value of $\rho_{u,v}^2(\mathbf{x})$  is of form
\begin{eqnarray*}
	&&\mathbb{E}[\rho_{u,v}^2(\mathbf{x})] = \sum_{j,j'\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cup \mathcal{I}(j')}(1-\mathbb{E}[x_t])\\&&
	=\sum_{j,j'\in \mathcal{J}(\mathcal{R},(u,v))}\beta_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cup \mathcal{I}(j')}(1-y_t),
\end{eqnarray*}
where $y_t = \mathbb{E}[x_t]$. Similarly, this approach can be used to compute $\mathbb{E}[\rho_{u,v}^k(\mathbf{x})]$, for $k>2$. The following lemma provides the tool to calculate $\mathbb{E}[\rho_{u,v}^k(\mathbf{x})]$, for $k>2$, which its proof is omitted due to similarity to previous calculations.
\begin{lemma}\label{lemma:induction}
	Given two polynomial functions $$f_1(\mathbf{x}) = \sum_{j\in \mathcal{J}}\alpha_j \prod_{t\in \mathcal{I}(j)}(1-x_t),  $$ $$f_2(\mathbf{x}) = \sum_{j\in \mathcal{J'}}\beta_j \prod_{t\in \mathcal{I}'(j)}(1-x_t),$$ where $\mathbf{x}\in \{0,1\}^n$, their product is of similar form and given by
	\begin{equation}
		(f_1 * f_2)(\mathbf{x}) = \sum_{j\in \mathcal{J},j'\in \mathcal{J}'}\alpha_j\beta_{j'} \prod_{t\in \mathcal{I}(j) \cup \mathcal{I}'(j')}(1-x_t).
	\end{equation}
\end{lemma}

Using Lemma \ref{lemma:induction}, we can then compute $\rho_{u,v}^k(\mathbf{x})$ using induction, and take its expected value. It follows
\begin{eqnarray*}
	&&\mathbb{E}[\rho_{u,v}^k(\mathbf{x})] = \sum_{j_1,j_2,\cdots,j_k\in \mathcal{J}(\mathcal{R},(u,v))}\prod_{i\in \{j_1,j_2,\cdots,j_k\}}\beta_i\times\\&&\prod_{t\in \cup_{j\in\{ j_1,j_2,\cdots,j_k\}} \mathcal{I}(j)}(1-y_t).
\end{eqnarray*}

Therefore, for a given $L$, we can compute an estimator for $\frac{\partial G}{\partial y_{vi}}$, denoted by $z'_{vi}$, with a tunable bias which is the function of $L$ and $\rho^*_{u,v}$.  It follows
\begin{equation}\label{eq:biased_est}
	z'_{vi} := \sum_{(u,v)\in E}\left(\sum_{k=0}^{L}\alpha^{(k)}_{u,v}\mathbb{E}[\rho_{u,v}^k|x_{vi}=0] - \sum_{k=0}^{L}\alpha^{(k)}_{u,v}\mathbb{E}[\rho_{u,v}^k|x_{vi}=1]\right).
\end{equation}
\begin{lemma}\label{lemma:bias}
	Given a set of continuous functions $\{C_{u,v}\}_{(u,v)\in E}$ where their first $L+1$ derivatives within their operating regime, $[0,1)$, are upperbounded by a finite constant, $W$, the bias of estimator $z':=[z'_{vi}]_{v\in V,i\in \mathcal{C}}$, where $z'_{vi}$ is  defined by \eqref{eq:biased_est}, is bounded by
	\begin{equation}\label{eq:bias}
		|\mathbb{E}\left[z|\mathbf{y}\right] -\triangledown G(\mathbf{y})| \leq\frac{W |V| |\mathcal{C}|}{(L+1)!}.
	\end{equation}
	\begin{proof}
		To compute the bias, we note that $\rho_{u,v}, \rho^*_{u,v} \in [0,1]$. Specifically, we assume $\rho_{u,v}, \rho^*_{u,v} \in [0,1)$. Hence, $|\rho_{u,v}- \rho^*_{u,v}| \leq 1$, and $C^{(L+1)}_{u,v}(\rho'_{u,v}) \leq \max \{C^{(L+1)}_{u,v}(\rho_{u,v}) ,C^{(L+1)}_{u,v}(\rho^*_{u,v}) \} <\infty$. In particular, let $ W =\max_{(u,v)\in E} C^{(L+1)}_{u,v}(\rho'_{u,v})$. Then, it is easy to compute the upperbound for the bias of $z'$, as given in \eqref{eq:bias}.
	\end{proof}
\end{lemma}
Using Lemma \ref{lemma:bias}, we can set
\begin{equation}
	B = \frac{W |V| |\mathcal{C}|}{(L+1)!}\label{eq:B}.
\end{equation}
Thus, by applying Algorithm \ref{alg:caching} with the deterministic biased estimator $z'$ given by \eqref{eq:biased_est}, we obtain the following optimality guarantee
\begin{equation}
	\mathbb{E}[G(\mathbf{y}_{K})] \geq (1-\frac{1}{e})G(\mathbf{y}^*) - DB - \frac{L}{2K}.
\end{equation}

\end{comment}


==> Kelly Cache Networks/model.tex <==
Motivated by applications such as ICNs \cite{jacobson2009networking}, CDNs \cite{borst2010distributed,dehghan2014complexity}, and peer-to-peer networks \cite{lv2002search}, we introduce Kelly cache networks. In contrast to classic Kelly networks, each node is associated with a cache of finite storage capacity. Exogenous traffic consisting of \emph{requests} is routed towards nodes that store objects; upon reaching a node that stores the requested object, a \emph{response} packet containing the object is routed towards the node that generated the request. As a result, content traffic in the network is determined not only by demand but, crucially, by how contents are cached. %Our model can also be seen as an extension of the cache networks presented in \cite{ioannidis2016adaptive}, incorporating queuing.
%
 \techrep{For completeness, we  review classic Kelly networks in Appendix~\ref{app:classickelly}.}{} An illustration highlighting the differences between Kelly cache networks, introduced below, and classic Kelly networks, can be found in Fig.~\ref{fig:kelly-classic}.
\begin{figure}
\includegraphics[width=0.49\columnwidth]{kelly-classic}\includegraphics[width=0.49\columnwidth]{kelly-caching}\\%\vspace*{-3em}
\begin{scriptsize} \hspace*{\stretch{1.3}}{(a) Kelly Network}\hspace*{\stretch{2}}
{(b) Kelly Cache Network}\hspace*{\stretch{1}}\end{scriptsize}\\
\caption{(a) Example of a Kelly network. Packets of class $r$ enter the network with rate $\lambda^r$,  are routed through consecutive queues over path $p^r$, and subsequently exit the network. (b) Example of a Kelly cache network. Each node $v\in V$ is equipped with a cache of capacity $c_v$. Exogenous requests of type $r$ for object $i^r$  enter the network and are routed  over a predetermined path $p^r$ towards the designated server storing $i^r$. Upon reaching an intermediate node $u$ storing the requested object $i^r$, a response packet containing the object is generated. The response is then forwarded towards the request's source in the reverse direction on path $p^r$. Request packets are of negligible size compared to response messages; as a result, we ignore request traffic and focus on queuing due to response traffic alone.} %: for example, for edge $(v,u)\in p^r$, response traffic contributes only to the load of reverse edge $(u,v)\in E$. }
\label{fig:kelly-classic}
\end{figure}

Although we describe Kelly cache networks in terms of FIFO M/M/1 queues, the product form distribution  (c.f.~\eqref{steadystate}) arises for many different service principles beyond FIFO (c.f.~Section 3.1 of \cite{kelly}) %. In short, incoming packets can be placed in random position within the queue according to a given distribution, and the (exponentially distributed) service effort can be split across different positions, possibly unequally;  both placement and service effort distributions are class-independent. This captures  a broad array of policies including FIFO,
including Last-In First-Out (LIFO) and processor sharing. All results we present extend to these service disciplines; we discuss %these and more
more extensions in Sec.~\ref{sec:beyond}.



\subsection{Kelly Cache Networks} 

\noindent\textbf{Graphs and Paths.} We use the notation $G(V,E)$ for a directed graph $G$ with nodes $V$ and edges $E\subseteq V\times V$. A directed graph is called \emph{symmetric} or \emph{bidirectional} if $(u,v)\in E$ if and only if $(v,u)\in E$. A \emph{path} $p$ is a sequence of adjacent nodes, i.e.,  $p=p_1,p_2,\ldots, p_K$ where $(p_{k},p_{k+1})\in E$, for all $1\leq i<K\equiv|p|$. A path is \emph{simple} if it contains no loops (i.e., each node appears once). We use the notation $v\in p$, where $v\in V$, to indicate that node $v$ appears in the path, and $e\in p$, where $e=(u,v)\in E$, to indicate that nodes $u$,$v$ are two consecutive (and, therefore, adjacent) nodes in $p$.  For $v\in p$, where $p$ is simple, we denote by $k_p(v)\in \{1,\ldots,|p|\}$ the position of node $v\in V$ in $p$, i.e., $k_p(v)=k$ if $p_k=v$.

%\begin{comment}
%\end{comment}
	%Jackson networks are a class of queuing networks where the equilibrium distribution has a simple product-form solution. In particular, an open Jackson network is a Jackson network, in which packets arrive from outside following some independent Poisson processes. Each arrived packet follows a route (a sequence of queues) independent of other packets, and leaves the network after it is served by the last queue along its path.
	


\noindent\textbf{Network Definition.} Formally,  we consider a Kelly network of M/M/1  FIFO queues, represented by a symmetric directed graph $G(V,E)$. As in classic Kelly networks, each edge $e\in E$ is associated with an M/M/1 queue with service rate $\mu_e$\footnote{We associate queues with edges for concreteness. Alternatively, queues can be associated with nodes, or both nodes and edges; all such representations lead to product form distributions \eqref{steadystate}, and all our results extend to these cases.}. In addition, each node has a cache that stores  objects of equal size from a set $\catalog$,  the \emph{object catalog}.  Each node $v\in V$ may store at most $c_v\in \naturals$  objects from $\catalog$ in its cache.  Hence, if $x_{vi} \in \{0,1\}$ is a binary variable indicating whether node $v\in V$ is storing object $i\in \catalog$, then 	
	%\begin{equation}\label{eq:cache_cap}
$		\sum_{i\in\catalog} x_{vi} \leq c_v,$ for all $v\in V. $
%	\end{equation}
We refer to $\mathbf{x}=[x_{vi}]_{v\in V, i\in \catalog} \in \{0,1\}^{|V||\catalog|}$ as the \emph{global placement} or, simply, \emph{placement} vector. We denote by
\begin{align}
\domain = \left\{\mathbf{x}\in \{0,1\}^{|V| |\catalog|}: \textstyle\sum_{i\in\catalog} x_{vi} \leq c_v, \forall v\in V \right \}, \label{domain}
\end{align}
the set of \emph{feasible} placements that satisfy the storage capacity constraints. %\eqref{eq:cache_cap}.
We assume that for every object $i\in\catalog$, there exists a set of nodes $\servers_i\subseteq V$ that \emph{permanently store} $i$. We refer to nodes in $\servers_i$ as \emph{designated servers} for $i\in \catalog$. We assume that designated servers store $i$ in permanent storage \emph{outside} their cache. Put differently, the aggregate storage capacity of a node is $c_v'=c_v+|\{i:v\in \servers_i\}|$, but only the non-designated slots $c_v$ are part of the system's design.

%Furthermore, the space restricted by the storage capacity constraints given in \eqref{eq:cache_cap}, is denoted by  $\mathcal{D}$. We note that the choice of $X$ can be made statically or dynamically in a randomized manner. For each object $i$, a fixed set of nodes, denoted by $\servers_i$, are designated to always store object $i$. We assume each source node has an external storage for storing its designated objects.	
%	\subsection{Request and Path Structure}
	
\noindent\textbf{Object Requests and Responses.}
Traffic in the cache network consists of two types of packets: \emph{requests} and \emph{responses}, as shown in  Fig.~\ref{fig:kelly-classic}(b).
 Requests for an object are always routed towards one of its designated servers, ensuring  that every request is satisfied. However, requests may terminate early: upon reaching any node that caches the requested object,  the latter generates a response carrying the object. This is forwarded  towards the request's source, following the same path as the request, in reverse. Consistent with prior literature \cite{ioannidis2016adaptive,ioannidis2017jointly}, %,mahdian2017mindelay},
 we treat request  traffic as negligible when compared to response traffic, which carries objects,  and henceforth focus only on queues bearing response  traffic.

 
Formally, a request and its corresponding response are fully characterized by (a)  the object  being requested, and (b) the path  that the request  follows. That is, for the set of requests $\demand$, a request $r\in \demand$ is determined by a pair $(i^r,p^r)$, where $i^r\in \catalog$ is the object being requested and $p^r$ is the path the request follows. 
Each request $r$ is associated with a corresponding Poisson arrival process with rate $\lambda^r\geq 0$, independent of other arrivals and service times.  We denote the vector of arrival rates by
%\begin{align}
$ \bm{\lambda} = [\lambda^r]_{r\in \demand} \in\reals_+^{|\demand|}.$
%\end{align}
%
For all $r\in \demand$, we assume that the path $p^r$ is well-routed \cite{ioannidis2016adaptive}, that is: (a) path $p^r$ is simple, (b) the terminal node of the path is a designated server, i.e., a node in $\servers_i$, and (c) no other intermediate node in $p^r$ is a designated server. As a result, requests are always served, and response packets (carrying objects) always follow a sub-path of $p^r$ in reverse towards the request source (namely, $p^r_1$). %As we assume that response packets are much larger than  request packets, we consider only the response traffic imposed on network queues. 

%We specify a request for a content object by the object and the path the request takes. That is, a request $r$ is a pair $(i,p)$ where $i\in \catalog$ and path $p$ is a sequence of nodes $\{p_1,p_2,\cdots,p_K\}$. In this example, $K:=|p|$ is the length of the path in nodes, denoted by $|p|$, and $p_k\in V$, for $k\in \{1,2,\cdots|p|\}$.
	
% When a request $r=(i,p)$ arrives at the requesting node $p_1$, it will be routed following path $p$, until it reaches a node which stores $i$. If no such node is found, $r$ reaches the designated source node $p_K$. In either way, a response is generated containing the content object, and is routed back over $p$ (or a part of $p$ in case of reaching a cache) in the reverse direction. 
	
%	We denote by $k_p(v)$ the index of node $v$ along path $p$. Moreover, we denote the upstream edges of node $v$ along all the paths of content $i$ which passes $v$ by $suc_{(i,P(i))}(v):= \{(u,w)\in E|\quad\exists p\in P(i), (w,u)\subseteq p, k_p(v) \leq k_p(w)\}$, where $P(i) = \{p:(i,p)\in \demand\}$. We assume each request is well-routed. That is, $p$ does not contain any loop, and there is exactly one designated source node for $i$ in $p$, which is always the ending node, $p_K$. 
	
%	Let $\demand$ be the set of all requests, in each of which its arrival follows an independent Poisson process with rate $\lambda_{(i,p)}>0$, $\forall (i,p)\in \demand$.

\noindent\textbf{Steady State Distribution.}	
Given an object placement $\mathbf{x}\in \domain$, the resulting system is  a multi-class Kelly network, with packet classes determined by the request set $\demand$. This is a Markov process over the state space determined by queue contents. In particular, let $n_e^r$ be the number of packets of class $r\in \demand$ in queue $e\in E$, and $n_e = \sum_{r\in \demand} n_e^r$ be the total queue size. The state of a queue $\mathbf{n}_{e}\in \demand^{n_{e}}$, $e\in E$, is the vector of length $n_{e}$ representing the class of each packet in each position of the queue. The \emph{system state} is then given by $\mathbf{n}=[\mathbf{n}_{e}]_{e\in E}$;  we denote by $\Omega$ the state space of this Markov process.

In contrast to classic Kelly networks, network traffic and, in particular, the load on each queue, 
 depend on placement $\mathbf{x}$. Indeed,  if $(v,u)\in p^r$ for $r\in \demand$, the arrival rate of responses of class $r\in \demand$ in queue $(u,v)\in E$ is:
\begin{align}\textstyle\lambda_{(u,v)}^r(\mathbf{x},\bm{\lambda}) =  \lambda^r \prod\limits_{k'=1}^{k_{p^r}(v)}(1-x_{p_{k'}^ri^r}),\label{lamr}\quad \text{for}~(v,u)\in p^r, \end{align}
i.e., responses to requests of class $r$ pass through edge $(u,v)\in E$ if and only if no node preceding $u$ in the path $p^r$ stores object $i^r$--see also Fig.~\ref{fig:kelly-classic}(b). As $\mu_{(u,v)}$ is the service rate of the queue in $(u,v)\in E$, % We assume the size of response packets is much bigger than the size of request packets, hence we only take into account the load (delay or number of packets) associated with the response packets in the queues. Let 
the  load on edge $(u,v)\in E$ is:
	 		\begin{align}
	 		%\rho_{(u,v)}(X) = \frac{1}{\mu_{(u,v)}} \sum\limits_{r\in\demand: (v,u)\in p^r}\lambda^r \prod\limits_{k'=1}^{k_{p^r}(v)}(1-x_{p_{k'}^ri^r}), \label{eq:rho_X}
	 		\textstyle\rho_{(u,v)}(\mathbf{x},\bm{\lambda}) = \frac{1}{\mu_{(u,v)}} \textstyle\sum_{r\in\demand: (v,u)\in p^r}\lambda^r_{(u,v)}(\mathbf{x},\bm{\lambda}). %\prod\limits_{k'=1}^{k_{p^r}(v)}(1-x_{p_{k'}^ri^r}), 
\label{eq:rho_X}
	 		\end{align} 
The Markov process $\{\mathbf{n}(t);t\geq 0\}_{t\geq 0}$ is positive recurrent when $\rho_{(u,v)}(\mathbf{x},\bm{\lambda})< 1$, for all $(u,v)\in E$ \cite{kelly,datanetworks}. Then, the steady-state distribution has a \emph{product form}, i.e.:
\begin{align}
\textstyle\pi(\mathbf{n}) =  \prod_{e\in E} \pi_e(\mathbf{n}_e), \quad \mathbf{n}\in \Omega,\label{steadystate}
\end{align}
 %yielding:
%\begin{align}
%\pi(\mathbf{n}) =  \prod_{e\in E} \pi_e(\mathbf{n}_e), \quad \mathbf{n}\in \Omega\label{steadystate}
%\end{align}  
where
%\begin{align}
$\textstyle\pi_e(\mathbf{n}_e) = (1-\rho_e(\mathbf{x},\bm{\lambda})) \prod_{r\in \demand:e\in p^r} \left(\frac{\lambda^r_e(\mathbf{x},\bm{\lambda}) }{\mu_e}\right)^{n_e^r},$% \label{eq:marg}
%\end{align}
and $\lambda_e^r(\mathbf{x},\bm{\lambda})$, $\rho_e(\mathbf{x},\bm{\lambda})$ are given by \eqref{lamr}, \eqref{eq:rho_X}, respectively.


%\si{add figure of requests and responses}
%	For a fixed content placement state $X$, the network model is reduced to a classic open Jackson network which is well-studied in \cite{kelly}, and \cite{datanetworks}. 
%	 		Let $N:=(N_{u,v})_{(u,v)\in E}$ be the vector state of number packets in the queues of the network, where $N_{u,v}$ is the number of packets in queue $(u,v)$, the Jackson's Theorem \cite{datanetworks} states that 
%	 			for a given request arrival vector $\demand$ and content placement vector $X$, for which $\rho_{u,v}(X)<1$, $\forall  (u,v)\in E$, he steady-state distribution follows
%	 				 			\begin{equation}
%	 				 			\pi_X(N) = \prod\limits_{(u,v)\in E} \pi_{X,u,v}(N_{u,v}),
%	 				 			\end{equation}
%	 				 			where 
%	 				 			$\pi_{X,u,v} (N_{u,v}) = (1- \rho_{u,v}(X))\rho_{u,v}(X)^{N_{u,v}}.$ 
%si{This is wrong. Not being careful with statements like that can get the paper rejected in no time.}
%	 		the following result for the steady-state distribution $\pi_X(N)$ for a given content placement vector $X$:
%	 		%	
%	 		\begin{theorem}(Jackson's Theorem \cite{datanetworks})
%	 			For a given request arrival vector $\demand$ and content placement vector $X$, for which $\rho_{u,v}(X)<1$, $\forall  (u,v)\in E$, we have
%	 			\begin{equation}
%	 			\pi_X(N) = \prod\limits_{(u,v)\in E} \pi_{X,u,v}(N_{u,v}),
%	 			\end{equation}
%	 			where 
%	 			$\pi_{X,u,v} (N_{u,v}) = (1- \rho_{u,v}(X))\rho_{u,v}(X)^{N_{u,v}}.$
%	 			\label{theorem:jackson}
%	 		\end{theorem}
	
	\noindent\textbf{Stability Region.} Given a placement $\mathbf{x}\in \mathcal{D}$,
	%Before solving for the problem in the next section, we first describe the stability region of the problem. We define the stability region of the problem as follows: for a given content placement vector $X\in\mathcal{D}$,
 a vector of arrival rates $\bm{\lambda} = [\lambda^r]_{r\in \demand}$ yields a stable (i.e., positive recurrent) system  
	if and only if $\bm{\lambda} \in \Lambda_{\mathbf{x}}$, where
	\begin{equation}
		\Lambda_{\mathbf{x}} := \{\bm{\lambda}: \bm{\lambda} \geq 0: \rho_e(\mathbf{x},\bm{\lambda})< 1, \forall e\in E \} \subset \reals_+^{|\demand|} ,
	\end{equation}
	where loads $\rho_e$, $e\in E$, are given by 
\eqref{eq:rho_X}. %Note that given $\mathbf{x}\in \mathcal{D}$, $\rho_{u,v}$ is linear in $\bm{\lambda}$;  hence, $\Lambda_{\mathbf{x}}$ is the interior of a convex polytope defined by linear inequality constraints. 
Conversely, given a vector $\bm{\lambda} \in \reals_+^{|\demand|}$,
\begin{align}
\domain_{\bm{\lambda}} = \{ \mathbf{x}\in \domain:  \rho_e(\mathbf{x},\bm{\lambda})< 1, \forall e\in E  \} \subseteq \domain \label{eq:stabledom}
\end{align}
is the set of feasible placements under which the system is stable. It is easy to confirm that, by the monotonicity of $\rho_e$ w.r.t.~$\mathbf{x}$, 
%\begin{align}
if $\mathbf{x}\in \domain_{\bm{\lambda}}$ and $\mathbf{x}'\geq \mathbf{x},$  then $\mathbf{x}'\in \domain_{\bm{\lambda}}$, %\label{eq:ldom}
%\end{align}
where the vector inequality $\mathbf{x}'\geq \mathbf{x}$ is component-wise.
In particular, if $\mathbf{0}\in D_{\bm{\lambda}}$ (i.e., the system is stable without caching), then $\domain_{\bm{\lambda}} = \domain$.
\begin{comment}
 the following properties hold:
\begin{align}
\text{if }X\geq X'\text{ then  }\Lambda_X \supseteq \Lambda_{X'},
\end{align} 
and
\begin{align}
\text{if }\lambda\geq \lambda'\text{ then  }\domain_\lambda \subseteq \domain_{\lambda'},
\end{align} 
where the above vector and matrix inequalities are component-wise.
\end{comment}
%it is equivalent to linear system $A(X)\lambda \prec 1$, where $A(X)=[A_{(i,p)\times (u,v)}(X)]_{(i,p)\in \demand, (u,v)\in E}$ is the matrix which its $(u,v)$-th row constitutes the coefficients of $\lambda_{(i,p)}$s' in $\rho_{u,v}(X)$, respectively. Therefore, the stability region under $X$ can be rewritten as
%	\begin{equation}
%		\Lambda_X = \{\lambda: \lambda \geq 0, A(X)\lambda \prec 1\}. 
%	\end{equation}	
\begin{comment}
	Treating placements as a design parameter, the overall system stability region is
	\begin{equation}
		\Lambda = \textstyle\bigcup_{X\in \domain} \Lambda_X.
	\end{equation}
	which, in general, may not be convex.
\end{comment}
     
	
	\subsection{Cache Optimization}\label{sec:mincost}

\begin{comment}
	Motivated by the Kelly's Theorem stated in previous section, we can now associate a cost function with the proposed network at its equilibrium. In particular, we consider a general class of convex and nondecreasing functions with respect to (w.r.t.) $\rho$'s for this purpose. Our goal here is to formulate an optimization problem which minimizes the associated network cost function subject to the stability region of the network. Due to the Jackson's Theorem, we know that the total network cost will be the total sum of costs associated with each queue. Hence, we associate a general nondecreasing convex cost function to each link, denoted by $C_{u,v}, \forall (u,v) \in E$. To translate the stability of the network into stability of the optimization problem, we require $C_{u,v}<\infty$, for $\rho_{u,v}(X)<1$, and $C_{u,v} \rightarrow \infty$, as $\rho_{u,v}(X)\rightarrow1^-$.
\end{comment}

	Given a Kelly cache network represented by graph $G(V,E)$, service rates $\mu_e$, $e\in E$, storage capacities $c_v$, $v\in V$, a set of requests $\demand$, and arrival rates $\lambda_r$, for $r\in \demand$, we wish to determine placements $\mathbf{x}\in \domain$ that optimize a certain design objective. In particular, we seek placements that are solutions to optimization problems of the following form:\\
	\begin{subequations}\label{opt:mincost}
{\hspace*{\stretch{1}} \textsc{MinCost} \hspace*{\stretch{1}} } 
	\vspace{-0.8em}	
		\begin{align}
	\textstyle \text{Minimize:}&\quad C(\mathbf{x}) = \textstyle\sum_{e\in E} C_e(\rho_e(\mathbf{x},\bm{\lambda})),\label{eq:obj}\\   
			\text{subj.~to:}&\quad \mathbf{x} \in\domain_{\bm{\lambda}} ,
	        \end{align} 
	\end{subequations}
where $C_e:[0,1)\to \reals_+$, $e\in E$, are positive \emph{cost} functions, $\rho_e:\domain\times \reals_+^{|\demand|}\to \reals_+$ is the load on edge $e$, given by \eqref{eq:rho_X}, and $\domain_{\bm{\lambda}}$ is the set of feasible placements that ensure stability, given by \eqref{eq:stabledom}. 
%
We make the following standing assumption on the cost functions appearing in \textsc{MinCost}:
\begin{assumption} For all $e\in E$, functions $C_e:[0,1)\to \reals_+$ are convex and non-decreasing on $[0,1)$. \label{as:conv}
\end{assumption}
Assumption \ref{as:conv} is natural; indeed it holds for many cost functions that often arise in practice. We list several examples:

\noindent\textbf{Example 1. Queue Size:} Under steady-state distribution~\eqref{steadystate}, the expected number of packets in queue $e\in E$ is given by
%\begin{align}
$\expect[n_e] = C_e(\rho_e) = \frac{\rho_e}{1-\rho_e},$% \label{eq:size}
%\end{align} 
which is indeed convex and non-decreasing for $\rho_e\in[0,1)$. Hence, the expected total number of packets in the system in steady state can indeed be written as the sum of such functions.

\noindent\textbf{Example 2. Delay:} From Little's Theorem \cite{datanetworks}, the expected delay experienced by a packet in the system is
%\begin{align}
$\expect[T] = \frac{1}{\|\bm{\lambda}\|_1} \sum_{e\in E} \expect[n_e],$
%\end{align}
where $\|\bm{\lambda}\|_1=\sum_{r\in\demand} \lambda^r$ is the total arrival rate, and $\expect[n_e]$ is the expected size of each queue. Thus, the expected delay can also be written as the sum of functions that satisfy Assumption~\ref{as:conv}. We note that the same is true for the sum of the expected delays per queue $e\in E$, as the latter are given by
%\begin{align}
$\expect[T_e] = \frac{1}{\lambda_e} \expect[n_e] = \frac{1}{\mu_e(1-\rho_e)},$
%\end{align}
which are also convex and non-decreasing in $\rho_e$.

\noindent\textbf{Example 3. Queuing Probability/Load per Edge:} In a FIFO queue, the \emph{queuing probability} is the probability of arriving in a system where the server is busy; this is given by $C_e(\rho_e)=\rho_e=\lambda_e/\mu_e$, which is again non-decreasing and convex.  
This is also, of course, the load per edge. By treating $1/\mu_e$ as the weight of edge $e\in E$, this setting recovers the objective  of \cite{ioannidis2016adaptive} as a special case of our model.

\noindent\textbf{Example 4. Monotone Separable Costs:} More generally, consider a state-dependent cost function $c:\Omega \to \reals_+$ that satisfies the following three properties: (1) it is separable across queues, (2) it depends only on queue sizes $n_e$, and (3) it is non-decreasing w.r.t.~these queue sizes. Formally, $c(\mathbf{n}) = \sum_{e\in E} c_e(n_e),$
where $c_e:\naturals\to \reals_+$, $e\in E$, are non-decreasing functions of the queue sizes. Then,
the steady state cost under distribution \eqref{steadystate} has precisely form \eqref{eq:obj} with convex costs, i.e.,
%\begin{align}
$\expect[c(\mathbf{n})] = \sum_{e\in E} C_e(\rho_e)$
%\end{align}
where $C_e:[0,1)\to\reals_+$ satisfy Assumption~\ref{as:conv}. 
 This follows from the fact that: \begin{align}
\!\!\!C_e(\rho_e) \!\equiv\! \expect[c_e(\mathbf{n})]\!=\! \textstyle c_e(0)+ \sum_{n=0}^{\infty}(c_e(n\!+\!1)\!-\!c_e(n)) \rho_e^n. \!\! \label{eq:power}
\end{align}
\techrep{The proof is in Appendix~\ref{app:convexity}.}{}

In summary, \textsc{MinCost} captures many natural cost objectives, while Assumption~\ref{as:conv} holds for \emph{any} monotonically increasing cost function that depends only on queue sizes.



\begin{comment}
	A good example for such a network cost function is total number of packets in the network, which is the sum of number of packets waiting for or under transmission at each queue. Further, since we are considering a stationary traffic arrival process, by Little's law, the number of packets in the network is proportional to the average packet delay. In this case, we will have
	$$C_{u,v}(X) = \frac{\rho_{u,v}(X)}{1-\rho_{u,v}(X)},\qquad \forall   (u,v) \in E,$$
	under $M/M/1$ queue model \cite{datanetworks}. Then, the aggregate network cost is given by
	\begin{equation}
		C(X) = \sum_{(u,v)\in E}C_{u,v}(X). \label{eq:C_X}
	\end{equation}
	
	Then, the cost minimization problem can be formulated as
	\begin{subequations}\label{opt:mincost}
		\begin{equation}
			\text{minimize } C(X)  
		\end{equation}
		\begin{equation} 
			\text{subject to: } X \in \mathcal{D}_1, 
		\end{equation}
	\end{subequations}
	where $\mathcal{D}_1$ is the set of vectors $X\in \mathbb{R}^{|V||\catalog|}$ satisfying
	\begin{subequations}
		\begin{equation}
			\sum_{i\in\catalog} x_{vi} \leq c_v,\qquad \forall v\in V, 
		\end{equation}
		\begin{equation}
			x_{vi} \in \{0,1\}, \qquad\qquad \forall v\in V, i\in \catalog,
		\end{equation}
	\end{subequations}
\end{comment}	

\begin{comment}
\subsection{Set Functions and Submodularity.} Given a finite set $\mathcal{X}$, a set function $f:\mathcal{X}\to \reals$ is called \emph{non-decreasing} if $f(S)\leq f(S')$ for all $S\subseteq S'\subseteq \mathcal{X}$, and \emph{non-increasing} if $-f$ is non-decreasing. Function $f$ is called \emph{submodular} if it satisfies the following \emph{diminishing returns} property: for all $S\subseteq S' \subseteq \mathcal{X}$, and all $x\in \mathcal{X}$,
\begin{align}f(S'\cup \{x\}) - f(S') \leq f(S\cup \{x\}) -f(S),  \label{submodular}\end{align}
A function is called \emph{supermodular} if $-f(S)$ is submodular (or, equivalently, \eqref{submodular} holds with the inequality reversed).

\end{comment}

\begin{table}[!t]
\begin{scriptsize}
\caption{Notation Summary}%\vspace*{-10mm}
\begin{tabular}{p{0.06\textwidth}p{0.38\textwidth}}
\hline
\multicolumn{2}{c}{\textbf{Kelly Cache Networks}}\\
\hline
$G(V,E)$ & Network graph, with nodes $V$ and edges $E$\\
$k_p(v)$ & position of node $v$ in path $p$\\
$\mu_{(u,v)}$ & Service rate of edge $(u,v)\in E$\\
$\demand$ & Set of classes/types of requests \\
$\lambda^r$ & Arrival rate of class $r\in \demand$ \\
$p^r$ & Path followed by  class $r\in \demand$ \\
$i^r$ & Object  requested by class $r\in \demand$ \\
$\catalog$ & Item catalog\\
$\mathcal{S}_i$ & Set of designated servers of $i\in \catalog$\\
$c_v$ & Cache capacity at node $v\in V$\\
$x_{vi}$ & Variable indicating whether $v\in V$ stores $i\in\catalog$ \\
$\mathbf{x}$ & Placement vector of $x_{vi}$s, in $\{0,1\}^{|V||\catalog|}$\\ %/relaxed variable $x_{vi}$\\
$\bm{\lambda}$ & Vector of arrival rates $\lambda^r$, $r\in \demand$\\
$\lambda_e^r$ & Arrival rate of class $r$ responses over edge $e\in E$\\
$\rho_e$ & Load on edge $e\in E$\\
$\Omega$ & State space\\
$\mathbf{n}$ & Global state vector in $\Omega$\\
$\pi(\mathbf{n})$ & Steady-state distribution of $\mathbf{n}\in \Omega$\\
$\mathbf{n}_e$ & State vector of queue at edge $e\in E$\\
$\pi_e(\mathbf{n}_e)$ & Marginal of steady-state distribution of queue $\mathbf{n}_e$\\
$n_e$ & Size of queue at edge $e\in E$\\
%\hline
%\multicolumn{2}{c}{\textbf{Kelly Cache Networks}}\\
%\hline
\hline
\multicolumn{2}{c}{\textbf{Cache Optimization}}\\
\hline
$C$ & Global Cost function\\
$C_e$ & Cost function of edge $e\in E$\\
$\domain$ & Set of placements $\mathbf{x}$ satisfying capacity constraints\\
$\mathbf{x}_0$ & A feasible placement in $\domain$\\
$F(\mathbf{x})$ & Caching gain of placement $\mathbf{x}$ over $\mathbf{x}_0$\\
$y_{vi}$ & Probability that $v\in V$ stores $i\in\catalog$ \\
$\mathbf{y}$ & Vector of marginal probabilities $y_{vi}$, in $\{0,1\}^{|V||\catalog|}$\\ %/relaxed variable $x_{vi}$\\
$G(\mathbf{y})$ & Multilinear extension under marginals $\mathbf{y}$\\
$\domain_{\bm{\lambda}}$ & Set of placements under which system is stable under arrivals $\bm{\lambda}$\\
$\tilde{\domain}$ & Convex hull of constraints of \textsc{MaxCG}\\
\hline
\multicolumn{2}{c}{\textbf{Conventions}}\\
\hline
$\supp(\cdot)$ & Support of a vector\\
$\conv(\cdot)$ & Convex hull of a set\\
$[\mathbf{x}]_{+i}$ & Vector equal to $\mathbf{x}$ with $i$-th coordinate set to 1 \\
$[\mathbf{x}]_{-i}$ & Vector equal to $\mathbf{x}$ with $i$-th coordinate set to 0 \\
$\mathbf{0}$ & Vector of zeros\\
\hline
\end{tabular}
\vspace*{-2em}
\end{scriptsize}
\end{table}



==> Kelly Cache Networks/related.tex <==
%There are several adaptive, distributed approaches determining how to populate caches under fixed routing. A simple, elegant, and ubiquitous algorithm is \emph{path replication}~\cite{cohen2002replication}, sometimes also referred to as ``leave-copy-everywhere'' (LCE) \cite{laoutaris2004meta}: once a request for an item reaches a cache, every downstream node receiving the response caches the item. Several variants of this principle exist. In ``leave-copy-down'' (LCD), a copy is placed \emph{only} in the node immediately preceding the cache storing the requested item \cite{laoutaris2004meta,laoutaris2006lcd}, while ``move-copy-down'' (MCD) also removes the present upstream copy. Probabilistic variants 
%have also been proposed \cite{psaras2012probabilistic}. To evict items, traditional eviction policies like Least Recently Used (LRU), Least Frequently Used (LFU), First In First Out (FIFO), and Random Replacement (RR) are typically used. Several  {works \cite{laoutaris2004meta,psaras2012probabilistic,wang2013optimal,rossini2014coupling,rossi2011caching} have studied the performance of these protocols and variants over a broad array of topologies. Despite the advantages of simplicity and elegance inherent in path replication, when targeting an optimization objective such as, e.g., minimizing total routing costs, path replication combined with all of the above eviction and replication policies is known to be arbitrarily suboptimal \cite{ioannidis2016adaptive}.
	
	
	% There is a vast literature on the performance of eviction policies like LRU, FIFO, LFU, etc., on a single cache, and the topic is classic \cite{dan1990approximate,achlioptas2000competitive,thomas1971analysis,flajolet1992birthday,gelenbe1973unified}. Nevertheless, the study of \emph{networks of caches} still poses significant challenges. A central problem is that, even if arriving traffic in an LRU cache is, e.g., Poisson, the \emph{outgoing} traffic is hard to describe analytically. Rosensweig et al.~\cite{rosensweig2013steady} study conditions under which path replication with LRU, FIFO, and variants, lead to an ergodic chain. 
	%  A significant breakthrough in this area has been the so-called \emph{Che approximation}  \cite{che2002hierarchical,fricker2012versatile}, which postulates that the hit rate of an LRU cache can be well approximated under the assumption that items stay in the cache for a constant time. This approximation is quite accurate in practice~\cite{fricker2012versatile}, and its success motivated extensive research in so-called \emph{time-to-live} (TTL) caches. In TTL caches, items stay in a cache for predetermined times, and are evicted when TTL timers expire. A series of recent works have focused on identifying how to set TTLs to (a) approximate the behavior of known eviction policies, (b) describe hit-rates in closed-form formulas~\cite{fofack2012analysis,che2002hierarchical,berger2014exact,dehghan2016utility,martina2014unified}. Despite these advances, none of the above works address issues of  routing cost minimization over multiple hops, which is our goal.
	
	% In their seminal paper~\cite{cohen2002replication} introducing path replication,  Cohen and Shenker also introduced the abstract problem of finding a content placement that minimizes routing costs. The authors show that path replication combined with a constant rate of evictions leads to an allocation that is optimal, in equilibrium, when nodes are visited through uniform sampling. %This is one of the few results on path replication's optimality---see also \cite{ioannidis2009absence}--though,
	%  Unfortunately, this optimality breaks down when uniform sampling is replaced by routing over arbitrary topologies \cite{ioannidis2016adaptive}.
	
%	Several papers have studied complexity and optimization issues of cost minimization as an offline caching problem under restricted topologies \cite{baev2008approximation,bartal1995competitive,fleischer2006tight,shanmugam2013femtocaching,applegate2010optimal,borst2010distributed}.  With the exception of \cite{shanmugam2013femtocaching}, these works model the network as a bipartite graph:  nodes generating requests connect directly to caches, and demands are satisfied a single hop, and do not readily generalize to arbitrary topologies. In general, the \emph{pipage rounding} technique of Ageev and Sviridenko~\cite{ageev2004pipage} (see also \cite{calinescu2007maximizing,vondrak2008optimal}) yields again a constant approximation algorithm in the bipartite setting, while approximation algorithms are also known for several variants of this problem~\cite{baev2008approximation,bartal1995competitive,fleischer2006tight, borst2010distributed}.


	Our approach is closest to, and inspired by, recent work by Shanmugam et al. \cite{femtocaching} and Ioannidis and Yeh  ~\cite{ioannidis2016adaptive}. 
 Ioannidis and Yeh consider a setting very similar to ours but without  queuing: edges are assigned a fixed weight, and the objective is a linear function of incoming traffic scaled by these weights. This can be seen as a special case of our model, namely, one where edge costs are linear (see also Sec.~\ref{sec:mincost}). Shanmugam et al.~\cite{femtocaching} study a similar optimization problem, restricted to the context of femtocaching. The authors show that this is an NP-hard, submodular maximization problem with matroid constraints. They provide a $1-1/e$ approximation algorithm based on a technique by Ageev and Sviridenko \cite{ageev2004pipage}: this involves maximizing a concave relaxation of the original objective, and rounding via pipage-rounding\cite{ageev2004pipage}. Ioannidis and Yeh show that the same approximation technique applies to more general cache networks with linear edge costs. They also provide a distributed, adaptive algorithm that attains an   $1-1/e$ approximation. The same authors  extend this framework to jointly optimize both caching and routing decisions \cite{ioannidis2017jointly}.

Our work can be seen as an extension of~\cite{ioannidis2016adaptive,femtocaching}, in that it incorporates queuing in the cache network. In contrast to both \cite{ioannidis2016adaptive} and \cite{femtocaching} however, costs like delay or queue sizes are highly non-linear in the presence of queuing. From a technical standpoint, this departure from linearity requires us to employ significantly different  optimization methods than the ones in \cite{ioannidis2016adaptive,femtocaching}. In particular, our objective \emph{does not admit a concave relaxation} and, consequently, the technique by Ageev and Sviridenko \cite{ageev2004pipage} used in \cite{ioannidis2016adaptive,femtocaching} \emph{does not apply}.  Instead, we must solve a non-convex optimization problem   directly  (c.f.~Eq.~\eqref{eq:nonconv}) using the so-called continuous-greedy algorithm.

 Several papers have studied the  cache optimization problems under restricted topologies \cite{baev2008approximation,bartal1995competitive,fleischer2006tight,applegate2010optimal,borst2010distributed}. These works model the network as a bipartite graph:  nodes generating requests connect directly to caches in a single hop.  The resulting algorithms do not readily generalize to arbitrary topologies. In general, the approximation technique of Ageev and Sviridenko~\cite{ageev2004pipage} applies to this bipartite setting, and additional approximation algorithms have been devised for several variants~\cite{baev2008approximation,bartal1995competitive,fleischer2006tight, borst2010distributed}. We differ   by (a)  considering a multi-hop setting, and (b) introducing queuing, which none of the above works considers.

%There have been multiple recent papers on distributed and adaptive caching strategies within the Information-Centric Networking (ICN) setting \cite{modeling,psaras2012probabilistic,caching2,ttlcachingDehgan,agebasedcachingMing,Carofiglio-LAC,kurose} with a variety of primary performance metrics taken into account, including cache hit probability \cite{modeling}, \cite{ttlcachingDehgan}, the reduction of the number of hops to retrieve the requested content \cite{psaras2012probabilistic}, and content download delay \cite{kurose}. Badov et al.~\cite{kurose} consider the content download delay as the performance metric of the interest and explored network	cache management and search policies that account for path-level	(content-server to content-requester) congestion and	file popularity in order to directly minimize 	content-download delay. 
	
%	Several recent works study caching and request forwarding  \emph{jointly}, in ICN networks \cite{yeh2014vip,mahdian2017mindelay}. Yeh et al, \cite{yeh2014vip} propose a unified framework for joint request forwarding and caching. They develop VIP, a set of distributed and dynamic request forwarding and caching algorithms, inspired by the backpressure routing algorithm, which adaptively maximizes the user demand rate the ICN network can satisfy. Mahdian and Yeh \cite{mahdian2017mindelay} study and formulate a relaxed cost minimization problem subject to joint request forwarding and caching within an ICN setting, based on a flow model framework inspired by the minimum-delay routing framework first introduced by Gallager \cite{gallager} for classic flow networks. They develop a distributed and online request forwarding and caching algorithm which attempts to reach a \emph{local} minimum of the network cost.
	
 % There is a vast literature on queuing networks with product-form steady-state distribution, following Jackson's original article \cite{jackson1957networks}, including several books by Kelly \cite{kelly}, Bertsekas and Gallager \cite{datanetworks}, and Nelson \cite{nelson}. Kelly \cite{kelly} extends the Jackson's single-class network of queues in several directions, including multi-class queues, and symmetric queues.
  
Submodular function maximization subject to matroid constraints appears in many important problems in combinatorial optimization; %~\cite{edmonds1970submodular,greedy2,vondrak2008optimal,greedy,calinescu2011};
for a brief review of the topic and applications, see \cite{krause2012} and \cite{goundan2007revisiting}, respectively. Nemhauser et al. \cite{greedy2} show that the greedy algorithm produces a solution  within 1/2 of the optimal.   Vondr\'ak \cite{vondrak2008optimal} and Calinescu et al. \cite{calinescu2011} show that the continuous-greedy algorithm produces a solution within $(1-1/e)$ of the optimal in polynomial time, which cannot be further improved \cite{nemhauser1978best}. 
%say something about curvature
In the general case, the continuous-greedy algorithm requires sampling to estimate the gradient of the so-called multilinear relaxation of the objective (see Sec.~\ref{sec:contgreed}). One of our main contributions is to show that \textsc{MaxCG}, the optimization problem we study here, exhibits additional structure: we use this  to construct a sampling-free estimator of the gradient via a power-series or Taylor expansion. To the best of our knowledge, we are the first to use such an expansion to eschew sampling; this technique may apply to submodular maximization problems beyond \textsc{MaxCG}.
 %Bian et al., \cite{Bian-CSM} applies the continuous greedy algorithm to optimize \emph{component-wise} convex functions with some optimality guarantees.

											

